Mathematical Information Retrieval: Search and Question Answering

Mathematical information is essential for technical work, but its creation, interpretation, and search are challenging. To help address these challenges, researchers have developed multimodal search engines and mathematical question answering systems. This book begins with a simple framework characterizing the information tasks that people and systems perform as we work to answer math-related questions. The framework is used to organize and relate the other core topics of the book, including interactions between people and systems, representing math formulas in sources, and evaluation. We close by addressing some key questions and presenting directions for future work. This book is intended for students, instructors, and researchers interested in systems that help us find and use mathematical information.

==> 00_test-macros.tex <==
\chapter*{TESTING MACROS}

\draftfigure
    {t}
    {Content for thee.}
    {Caption for thee.}
    {df}

\drafttable
    {t}
    {Content for thee and thine.}
    {Caption for thee and thine.}
    {dt}

% Author comment boxes
\axa{TEST}
\bm{TEST}
\rz{TEST}

This is a pair of references, to \reffig{df}
and \reftab{dt}.

\oursection{A Labeled Macro Section}{sec:lsec}

\oursubsection{A Labeled Section}{sec:subsec}

\ourfigure
    {!b}
    {\includegraphics{essence_logo}}
    {CAPTION}
    {fig:x}

A reference to an in-place table \reftab{tab:x}.

\ourtable
    {h}
    {\begin{tabular}{c c} \hline a & b \\ c & d \\ \hline \end{tabular}}
    {TAB-CAPTION}
    {tab:x}

\oursubsection{Referencing Tables, Figures, and Sections}{sec:refs}

A reference to a `real' figure using our macro: \reffig{fig:x}.

Here is are references to \refsec{sec:lsec} and \refsec{sec:subsec}.

==> INR-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}

\journalchiefeditor{Maarten de Rijke}{University of Amsterdam \\ and Ahold Delhaize\\The Netherlands}
\journalchiefeditor{Yiqun Liu}{Tsinghua University\\China}
\journalchiefeditor{Diane Kelly}{University of Tennessee\\USA}



\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Barbara Poblete}{University of Chile}
\journaleditor{Claudia Hauff}{Delft University of Technology}
\journaleditor{Doug Oard}{University of Maryland}
\journaleditor{Ellen M. Voorhees}{National Institute of Standards and Technology}
\journaleditor{Fabrizio Sebastiani}{Consiglio Nazionale delle Ricerche, Italy}
\journaleditor{Hang Li}{Bytedance Technology}
\journaleditor{Isabelle Moulinier}{Capital One}
\journaleditor{Jaap Kamps}{University of Amsterdam}
\journaleditor{Jimmy Lin}{University of Waterloo}
\journaleditor{Leif Azzopardi}{University of Glasgow}
\columnbreak
\journaleditor{Lynda Tamine}{University of Toulouse}
\journaleditor{Mark Sanderson}{RMIT University}
\journaleditor{Rodrygo Luis Teodoro Santos}{Universidade Federal de Minas Gerais}
\journaleditor{Ruihua Song}{Renmin University of China}
\journaleditor{Ryen White}{Microsoft Research}
\journaleditor{Shane Culpepper}{RMIT}
\journaleditor{Soumen Chakrabarti}{Indian Institute of Technology}
\journaleditor{Xuanjing Huang}{Fudan University}
\journaleditor{Zi Helen Huang}{University of Queensland}
\end{multicols*}
\end{editorialboard} 

==> INR-journaldata.tex <==
 \definecolor{palatinapurple}{rgb}{0.41, 0.16, 0.38}
\colorlet{INRcolor}{palatinapurple}   %new color names can be defined before use
\journalcolor      {INRcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Information Retrieval}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {INR}
\journalurl        {http://www.nowpublishers.com/INR}
\journalissnprint  {1554-0669}
\journalissnonline {1554-0677}
\journaldoi        {10.1561/15}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Information Retrieval publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Applications of IR}
\item{Architectures for IR}
\item{Collaborative filtering and recommender systems}
\item{Cross-lingual and multilingual IR}
\item{Distributed IR and federated search}
\item{Evaluation issues and test collections for IR}
\item{Formal models and language models for IR}
\item{IR on mobile platforms}
\item{Indexing and retrieval of structured documents}
\item{Information categorization and clustering}
\item{Information extraction}
\item{Information filtering and routing}
\item{Metasearch, rank aggregation and data fusion}
\item{Natural language processing for IR}
\item{Performance issues for IR systems, including algorithms, data structures, optimization techniques, and scalability}
\item{Question answering}
\item{Summarization of single documents, multiple documents, and corpora}
\item{Text mining}
\item{Topic detection and tracking}
\item{Usability, interactivity, and visualization issues in IR}
\item{User modelling and user studies for IR}
\item{Web search}
\end{itemize}
\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Information Retrieval, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 5 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> INR-seriespage.tex <==
\vspace{12pt}

\noindent \textit{Extracting, Mining and Predicting Users’ Interests from Social Media}\\
Fattane Zarrinkalam, Stefano Faralli, Guangyuan Piao and Ebrahim Bagheri\\
ISBN: 978-1-68083-738-4\\

\noindent \textit{Knowledge Graphs: An Information Retrieval Perspective}\\
Ridho Reinanda, Edgar Meij and Maarten de Rijke\\
ISBN: 978-1-68083-728-5\\

\noindent \textit{Deep Learning for Matching in Search and Recommendation}\\
Jun Xu, Xiangnan He and Hang Li \\
ISBN: 978-1-68083-706-3\\

\noindent \textit{Explainable Recommendation: A Survey and New Perspectives}\\
Yongfeng Zhang and Xu Chen\\
ISBN: 978-1-68083-658-5\\

\noindent \textit{Information Retrieval: The Early Years}\\
Donna Harman\\
ISBN: 978-1-68083-584-7\\

\noindent \textit{Bandit Algorithms in Information Retrieval}\\
Dorota Glowacka\\
ISBN: 978-1-68083-574-8\\

\noindent \textit{Neural Approaches to Conversational AI}\\
Jianfeng Gao, Michel Galley and Lihong Li\\
ISBN: 978-1-68083-552-6\\

\noindent \textit{An Introduction to Neural Information Retrieval}\\
Bhaskar Mitra and Nick Craswell\\
ISBN: 978-1-68083-532-8

==> NOWFnT-data.tex <==
\newcommand\nowfnt@publicationaddress
 {%
  \textit{Published, sold and distributed by:}\\
  now Publishers Inc.\\
  PO Box 1024\\
  Hanover, MA 02339\\
  United States\\
  Tel.\ +1-781-985-4510\\
  www.nowpublishers.com\\
  sales@nowpublishers.com%
  \par
  \textit{Outside North America:}\\
  now Publishers Inc.\\
  PO Box 179\\
  2600 AD Delft\\
  The Netherlands\\
  Tel.\ +31-6-51115274
 }

\newcommand\nowfnt@legalrightstext
 {%
  All rights reserved. No part of this publication may be
  reproduced, stored in a retrieval system, or transmitted in any form or by any means, mechanical, photocopying, recording or otherwise, without prior written permission of the publishers.
  \par
  Photocopying. In the USA: This journal is registered at the Copyright  Clearance Center, Inc., 222 Rosewood Drive, Danvers, MA 01923.  Authorization to photocopy items for
  internal or personal use, or the internal or personal use of specific  clients, is granted by now Publishers Inc for users registered with the Copyright Clearance Center (CCC).
  The `services' for users can be found on the internet at:
  www.copyright.com
  \par
  For those organizations that have been granted a photocopy license, a separate system of payment has been arranged. Authorization does not extend to other kinds of copying, such as that for general distribution, for advertising or promotional purposes, for creating new collective works, or for resale.  In the rest of the world:
  Permission to photocopy must be obtained from the copyright
  owner. Please apply to now Publishers Inc., PO Box 1024, Hanover, MA 02339, USA; Tel. +1 781 871 0245; www.nowpublishers.com; sales@nowpublishers.com
  \par
  now Publishers Inc. has an exclusive license to publish this
  material worldwide. Permission to use this content must be obtained from the copyright license holder. Please apply to now Publishers, PO Box 179, 2600
  AD Delft, The Netherlands, www.nowpublishers.com; e-mail:
  sales@nowpublishers.com}

\newcommand\nowfnt@printedoninfotext
 {%
  {%
   %
  }%
 }

\newcommand\nowfnt@howtocitetext
 {%
  The preferred citation for this publication is\par
  {%
   \raggedright
   \useissuedata{copyrightowner}.
   \emph{\nowfnt@articletitle}.
   \printjournaltitleprefix \usejournaldata{title}, vol.~\useissuedata{volume}, no.~\useissuedata{issue}, pp.~\useissuedata{firstpage}--\useissuedata{lastpage},
   \useissuedata{pubyear}.%
  }%
 }


\newcommand\nowfnt@copyrightlinetext
 {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} \useissuedata{copyrightowner}}

\newcommand\nowfnt@NOWcopyrightlinetext  %for wrapper
  {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} Now Publishers Inc}

\newcommand\nowfnt@sourceintro{%
 The content of the book was originally published in  }

\newcommand\nowfnt@sourcepunct{.}

\newcommand\nowfnt@prohibitiontext{This article may be used only for the purpose of research, teaching, and/or private study. Commercial use or systematic downloading (by robots or other automatic processes) is prohibited without explicit Publisher approval.}

\newcommand\nowfntstandardcitation{\nowfnt@authorlist@toc\ (\nowfnt@issuepubyear), \enquote{\nowfnt@articletitle}, \nowfnt@journaltitle: Vol. \nowfnt@issuevolume, No. \nowfnt@issueissue, pp \nowfnt@issuefirstpage--\nowfnt@issuelastpage. DOI: \nowfnt@issuedoi.}

%Title for the series pages.
\newcommand\nowfnt@seriespagetitle{\section*{Other titles in \nowfnt@journaltitle}}

==> ch0-index-test.tex <==
\index{Another item}
\index{Another item B}
\index{Another item C}
\index{Another item D}
\index{Another item E}
\index{Another item F}
\index{Another item G}
\index{Another item H}
\index{Another item H1}
\index{Another item H2}
\index{Another item H3}
\index{Another item H4}
\index{Another item H5}
\index{Another item H6}
\index{Another item H7}
\index{Another item H8}
\index{Another item H9}
\index{Another item H10}
\index{Another item H11}
\index{Another item H12}
\index{Another item H13}
\index{Another item H14}
\index{Another item H10}
\index{Another item H20}
\index{Another item H30}
\index{Another item H40}
\index{Another item H50}
\index{Another item H60}
\index{Another item H70}
\index{Another item H80}
\index{Another item H90}
\index{Another item H100}
\index{Another item H110}
\index{Another item H120}
\index{Another item H130}
\index{Another item H140}
\index{Another item H110}
\index{Another item H120}
\index{Another item H130}
\index{Another item H140}
\index{Another item H150}
\index{Another item H160}
\index{Another item H170}
\index{Another item H180}
\index{Another item H190}
\index{Another item H1100}
\index{Another item H1110}
\index{Another item H1120}
\index{Another item H1130}
\index{Another item H1140}
\index{Another item H1110}
\index{Another item H1120}
\index{Another item H1130}
\index{Another item H1140}
\index{Another item H1150}
\index{Another item H1160}
\index{Another item H1170}
\index{Another item H1180}
\index{Another item H1190}
\index{Another item H1100A}
\index{Another item H1110B}
\index{Another item H1120C}
\index{Another item H1130D}
\index{Another item H1140E}
\index{Another item H1110F}
\index{Another item H1120G}
\index{Another item H1130H}
\index{Another item H1140I}
\index{Another item H1150J}
\index{Another item H1160K}
\index{Another item H1170L}
\index{Another item H1180M}
\index{Another item H1190N}

\index{Formula Representations!Symbol Layout Tree (SLT)} 
\index{Formula Representations!Operator Tree (OPT)}
\index{Formula Representations!Baseline Structure Tree (BST)}

==> ch0-main-nowbook.tex <==
\PassOptionsToClass {book,biber}{nowfnt}
\input {ch0-main}


==> ch0-main-nowchapter.tex <==
\PassOptionsToClass {chapter,biber}{nowfnt}
\input {ch0-main}


==> ch0-main-nowebook.tex <==
\PassOptionsToClass {ebook,biber}{nowfnt}
\input {ch0-main}


==> ch0-main-nowechapter.tex <==
\PassOptionsToClass {echapter,biber}{nowfnt}
\input {ch0-main}


==> ch0-main-nowplain.tex <==
\PassOptionsToClass {plain,biber}{nowfnt}
\input {ch0-main}


==> ch0-main-nowsample.tex <==
\PassOptionsToClass {sample,biber}{nowfnt}
\input {ch0-main}


==> ch0-preface-draft.tex <==
\chapter*{Preface}
\addcontentsline{toc}{chapter}{Preface}
\textbf{This is an early draft of the book.} All chapters are now complete, but are likely to be revised in a later version.

If you have any comments questions, please feel free to contact the authors at \href{mailto:rxzvcs@rit.edu}{rxzvcs@rit.edu}.

~\\

\noindent Best wishes,\\

\noindent Richard Zanibbi\\
Behrooz Mansouri\\
Anurag Agarwal

\forceline

\scalebox{0.25}{
\includegraphics{figures/Book-Organization.pdf}
}

==> ch3-task-examples.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%
% EXAMPLES of retrieval tasks
%%%%%%%%%%%%%%%%%%%%%%%%%%
%\citep{10.1007/978-3-031-13643-6_20}
%Then, GPT-3 completes the text and produces an answer of up to 570 tokens:
%\begin{Verbatim}[commandchars=\\\{\}]
%  Q: What does it mean for a matrix to be Hermitian?
%
%  A: \textbf{A matrix is Hermitian if it is equal to its transpose conjugate.}
%\end{Verbatim}
%If the answer is longer than the maximum of 1,200 Unicode characters, the system retries until the model has produced a sufficiently short answer.

\begin{myexample}{Formula Search Tasks}{eg:ftasks}

\begin{scriptsize}

	%~\\
	
\flushleft 
\paragraph{\mbox{Formula similarity search}}
\centering 


%\flushleft
%\fheader{Formula similarity search} 
%\linebreak
%\centering

    \begin{tabular}{c | c  l }
       % \toprule
             \textbf{Query} & \multicolumn{2}{c}{\textbf{Result}}\\
            \midrule
            $y=\frac{a+bx}{b-x}$  & 1 & $y=\frac{a+bx}{c+x}$ 	\\
            & 2 & $y=a+bx$ 			\\
            & 3 & $y=\frac{a-bx}{c-x}$ 	\\
            & 4 & $y=\frac{a+bx}{x+c}$ 	\\
            & 5 & $g(x)=\frac{x}{x-a}$ 		\\   
            & \vdots & \vdots\\
      \bottomrule
    \end{tabular}   
    
%\flushleft
\paragraph{Formula similarity search w. query wildcards (?w)}
%\centering

    \begin{tabular}{l | l l }
    	%\toprule
         
        \textbf{Query} & \multicolumn{2}{l}{\textbf{Result}}\\ 
         
         \hline
         ~\\
         \scriptsize
        $
        \displaystyle
        \frac{\mathbf{?f}(\mathbf{?v}+\mathbf{?d})-\mathbf{?f}(\mathbf{?v})}{\mathbf{?d}}
        $ 
        
        &
        
        1
        
        &
        
        $
        \displaystyle
        g'(cx)=\lim_{h\to 0}\frac{\mathbf{g}(\mathbf{cx}+\mathbf{h})-\mathbf{g}(\mathbf{cx})}{\mathbf{h}}
        $\\
        & \vdots & \vdots \\
        \bottomrule
    \end{tabular}


%\flushleft
\paragraph{Contextualized formula search: MSE$^*$ answer posts}
%\centering

\begin{tabular}{p{1.5in} | c p{1.5in} }
       %\toprule
            \textbf{Query} & \multicolumn{2}{l}{\textbf{Result}}\\ %Rank & Formula \\
            \hline
    


%{\sc Formula Query inside a Math Question(Topic B.4)} 

\textcolor{gray}{
I have the sum}
$$
\boxed{
\displaystyle
\sum_{k=0}^{n} {n\choose k} k 
}
$$
\textcolor{gray}{
know the result is $n^2-1$ but I don't know how you get there. How does one even begin to simplify a sum like this that has binomial coefficients.}

&

1

& 
\textcolor{gray}{
\vdots 
\linebreak
which can be obtained by manipulating the second derivative of 
}
$$
\boxed{
\displaystyle
 \sum_{k=0}^n {n\choose k} z^k
}
$$
\textcolor{gray}{
and let $z = p/(1-p)$
}
\linebreak
\vdots
\\

%\hline
&

2

&
%{\sc Non-Relevant}

\textcolor{gray}{
Yes, it is in fact possible to sum this. The answer is 
}
$$
\boxed{
\displaystyle
\sum_{k=0}^n{n\choose k}{m\choose k}={m+n\choose n}
}
$$
\textcolor{gray}{
assuming that $n\leq m$. This comes from the fact that 
}

\vdots
\\

\bottomrule
\end{tabular}

~\\
*MSE: Math Stack Exchange
\end{scriptsize}
\end{myexample}



%%%%%%%%%%%%%%%%%%%%%%%%%%%
% FORMULA + TEXT TASKS
%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{myexample}{Math-Aware Search and Question Answering Tasks}{eg:ft_tasks}

\scriptsize

\flushleft
\section*{Ad-hoc retrieval: MSE$^*$ answer posts}
\centering

\begin{tabular}{p{1.5in} | c p{1.5in} }
       %\toprule
            \textbf{Query} & \multicolumn{2}{l}{\textbf{Result}}\\ %Rank & Formula \\
            \hline
    


%{\sc Formula Query inside a Math Question(Topic B.4)} 


I have the sum 
%\mbox{~~~~~~~~~~~~~~~~} 
%\linebreak
%\fbox{
$$\sum_{k=0}^{n} {n\choose k} k$$
%}
know the result is $n^2-1$ but I don't know how you get there. How does one even begin to simplify a sum like this that has binomial coefficients.
&

1

& 

\vdots  
which can be obtained by manipulating the second derivative of 
$$
 \sum_{k=0}^n {n\choose k} z^k
$$
and let $z = p/(1-p)$
\linebreak
\vdots
\\

%\hline
&

2

&
%{\sc Non-Relevant}
Yes, it is in fact possible to sum this. The answer is 
$$
\sum_{k=0}^n{n\choose k}{m\choose k}={m+n\choose n}
$$
assuming that $n\leq m$. This comes from the fact that 
\linebreak
\vdots
\\

\bottomrule
\end{tabular}


\flushleft
\section*{Math Q/A: Written response}
\centering

\begin{tabular}{p{1.5in} | p{2in} }
       %\toprule
            \textbf{Query} & \textbf{Result}\\ %Response only \\
            \midrule
%\citep{10.1007/978-3-031-13643-6_20}
%Then, GPT-3 completes the text and produces an answer of up to 570 tokens:

 What does it mean for a matrix to be Hermitian?
 
 & 

 A matrix is Hermitian if it is equal to its transpose conjugate.

%If the answer is longer than the maximum of 1,200 Unicode characters, the system retries until the model has produced a sufficiently short answer.
\\
	\bottomrule
\end{tabular}


\flushleft
\section*{Math word problem Q/A: Equation \& value response}
\centering

    \begin{tabular}{p{2.25in}  |   l  l }
       % \toprule
             \textbf{Query} & \multicolumn{2}{c}{\textbf{Result}}\\
             & Equation & Solution\\
             \midrule
Sarah has 5 pens, David has 3 pens. How many pens do they have? & $x=5+2$ & 8\\ 
\hline
~\\
%\hline
Find two consecutive integers whose sum is 7. & $x+(x+1)=7$ & 3, 4\\
\bottomrule
\end{tabular}

~\\
\flushleft
*MSE: Math Stack Exchange
\end{myexample}


==> ch5-formula+text-search.tex <==
%\chapter{Searching with Formulas and Text}
\chapter{Math-Aware Search}
\label{c-formula-text-search} % a label for the chapter, to refer to it later

% \section{Source Annotations}

% TBD...

%\section{Queries Combining Formulas and Text}
%[+QA]
%Math-aware search using text and formula can be considered as a part of the broader task known as multimodal information retrieval. Multimodal information retrieval involves the integration and use of multiple types of data or input modalities to retrieve information. In the context of mathematical information retrieval, these modalities include traditional text-based queries and mathematical formulas. By leveraging multimodal information retrieval techniques, search engines can provide more precise and comprehensive results. This capability is particularly crucial in fields like mathematics, where the interplay between textual descriptions and formal symbolic representations is essential for conveying and understanding complex concepts. Thus, incorporating both modalities, text, and formulas, enhances the ability to locate useful information in the mathematical literature.

As previously discussed in Chapter 2, the information conveyed by a formula generally depends heavily upon its surrounding textual context to define variables, operations, and other pertinent information not represented in the formula itself.
On their own, formulas primarily convey the operation hierarchy in an expression, and even then assuming that the set of operations and their interactions is known to the reader. 

In this chapter we consider three tasks that require using the interaction between formulas and text in sources:
\begin{compactenum}
\item math-aware search
\item math question answering
\item theorem proving
\end{compactenum}
Our treatment of theorem proving here is largely focused on applications of dense embeddings and search in the context of supporting premise selection and proof generation.

A common theme across these tasks is the importance of representations used for formulas and text both for original data from sources, and the choice of patterns used to represent mathematical information for computation, whether symbolically in OPTs, inverted index tables, or logical expressions, or as continuous dense vectors embedding the same chosen patterns. 
These chosen data structures serve as information sources that constrain and guide subsequent \emph{applications} of information embedded in algorithms used to complete tasks (\eg to answer a math question from a generated OPT or state representation for sentences in a word problem).

We will also see a recurring role for different forms of annotation of information sources, such as command tokens being inserted in text tokens for transformer inputs, and adding examples of step-by-step answers to questions before a question we want  to put to a large language model (LLM).
Converting questions in natural language to an OPT or other representation is a form of annotation of its own, adding a new representation for mathematical information in the question.
We will return to our information task models from Chapter 1 again later. 





%In this chapter we again focus on the search and answer generations of our system digram (see \reffig{fig:ch4overview}). [...]

%\ourfigscaled
%	{!t}
%	{0.6}
%	{figures/MathAwareSearch/MathTextQueryExamples}
%	{Examples of queries combining math formulas and text. Ad-hoc queries combine keywords and formulas in a manner similar to what one might
%	submit to a search engine. Excerpt queries ... ??? These are excerpts -- some might be written from scratch.}
%	{fig:optText}

%Again, harken back to chs 5-7. This may not be very long, but makes how queries appear explicit, rather than implied.



\section{Test collections for math-aware search}%: Tasks and Evaluation}


\ourtable
	{!t}
	{
		\scriptsize	
		\begin{tabular}{p{1.15in}   p{0.8in} p{0.8in} p{0.75in} p{0.75in} p{0.75in} }
		
		\toprule
		\textbf{Task \& }		  		&  \textbf{Collection of}	&		&		& \textbf{Effectiveness}\\
		\textbf{Test Collection}	& \textbf{Sources} & \textbf{Queries} & \textbf{Results} & \textbf{Metrics}\\
		\hline
		
		% ~\\
		% \multicolumn{5}{l}{ {\bf Formula Search} }\\
		% \midrule

		% NTCIR-10 \hfill(2013)	& 	arXiv papers 	 &  Organizers$^w$ & 	F in paper & mAP, P@\{5,10,hit\}\\
		% NTCIR-11 \hfill(2014)	& 	Wikipedia		 &  Individual Wiki \linebreak F (known item) 	& F in articles & mRR\\
		% NTCIR-12 \hfill(2016)	& 	Wikipedia$'$ & \mbox{Organizers}$^w$ &  F in articles 		& P@\{5,10,15,20\}, Bpref\\

		% \hline
		% ARQMath-1 \hfill(2020)	& 2018 MSE As & 2019 MSE Qs 	& F in MSE As & nDCG$'$, mAP$'$, P$'$@10 \\%\emph{*Contextualized}\\
		% ARQMath-2 \hfill(2021)	&  	& 2020 MSE Qs 	& 	 &  \\%\emph{*Contextualized}\\
		% ARQMath-3 \hfill(2022)	& 	 & 2021 MSE Qs 	& 	 &  \\%\emph{*Contextualized}\\
		% \hline
		% \underline{AccessMath}$^\dagger$ \hfill (2018) & \mbox{Videos +} \LaTeX{}~notes & \mbox{Image~region} \linebreak or~\LaTeX{} & Image regions or \LaTeX{} form. & R@10, mRR@10\\
		% %\midrule
		
		%~\\
		%\multicolumn{5}{l}{ {\bf Math-Aware Search (Ad-Hoc Retrieval)  } }\\
		%\midrule
		MREC 	\hfill(2011) 	& arXiv papers 		& $--$ & $--$ & $--$\\
		CUMTC 	\hfill(2015) 	& \mbox{arXiv papers} \linebreak (MREC data) & MathOverflow Qs & Papers & mAP\\
		%\hline
		\textbf{NTCIR-10} \hfill(2013)	& arXiv papers & Organizers$^w$ & Papers & mAP, P@\{5,10,hit\}\\
		NTCIR-11 \hfill(2014)	& \mbox{arXiv frags.} & Organizers$^w$ & Paper frags. & mAP, P@\{5,10,hit\}, Bpref\\
		NTCIR-12 \hfill(2016)	& \mbox{1. arXiv frags.} \linebreak 2. Wikipedia$'$ & \mbox{1. Organizers$^w$} \linebreak \mbox{2. Organizers$^w$} & \mbox{1. Paper frags.} \linebreak \mbox{2. Wiki articles} & P@\{5,10,15,20\}\\
		%\hline
		\textbf{ARQMath-1} \hfill(2020)	& 2018 MSE As & 2019 MSE Qs & F in MSE As &  nDCG$'$, mAP$'$, P$'$@10 \\%\emph{*Contextualized}\\
		ARQMath-2 \hfill(2021)	&  & 2020 MSE Qs & 	 &  \\%\emph{*Contextualized}\\
		ARQMath-3 \hfill(2022)	&  & 2021 MSE Qs &  	&  \\%\emph{*Contextualized}\\
		\underline{Cross-Math}$^\dagger$ \hfill (2024)	&  & \mbox{ARQMath 1-3 Qs} (4 languages) & 	  & P$'$@10, nDCG$'$@10\\
		\midrule
		
		% ~\\
		% \multicolumn{5}{l}{{\bf Reference Retrieval for Theorem Proving}} \\
		% \midrule
		% \mbox{NATURALPROOFS} \linebreak (2021) & \mbox{Proof references:} ProofWiki, \linebreak Stacks, Textbks.  & Theorem	& \mbox{Ref set/sequence} in proof & mAP, R@k, edit distance, BLEU\\
		% \bottomrule		
		\end{tabular}\\
		\scriptsize
		\textbf{F:} Formula; \textbf{As}: Answers; \textbf{Qs}: Questions; \textbf{MSE:} Math Stack Exchange
		\linebreak
		$^w${\textbf{Wildcard symbols} in at least some query formulas} 
		\linebreak
		 $^\dagger$Cross-modal or cross-language retrieval; \textbf{frags.}: Fragments (roughly paragraphs)
	}
	{Math-Aware Search Tasks and Test Collections}
	{tab:mas-colls}


A math-aware search engine supports search in a collection of sources using both formulas and keywords. 
This task distinguishes itself from isolated and contextualized formula search tasks by representations used for queries, and the associated information needs. 
%For formula search, information needs tend be focused on individual formulas.
Math-aware search tasks range from the simple ad-hoc query ``$a^2+b^2=c^2$ proof'' to full mathematical questions expressed using formulas and text. 
As with formula search, currently the primary standard test collections for this task are NTCIR and ARQMath. Additional details and comparison of these collections can be found elsewhere \citep{evalarxiv}. 
Test collections for math-aware search are summarized in \reftab{tab:tasks-sources}.

\textbf{MREC and CUMTC:} The first collection with annotated formulas that we are aware of goes back to 2011, when the Mathematical REtrieval Collection\footnote{\url{https://mir.fi.muni.cz/MREC/index.html}} (MREC) \citep{livska2011web} data set was introduced. MREC consists of 439,423 scientific documents from arXiv with more than 158 million formulae with MathML annotations. 
%MREC was a collection without any topics for measuring effectiveness. MREC was mostly used to study the efficiency of formula search systems. 
Four years later, the Cambridge University MathIR Test Collection (CUMTC) \citep{stathopoulos2015retrieval} built on MREC, adding 160 test topics derived from 120 MathOverflow discussion threads. This was one of the first attempts to use math community question-answering websites for producing real-world topics rather than topics created by shared task organizers. CUMTC topics were selected from question excerpts from 120 threads. These threads have at least one citation to the MREC collection in their accepted answer.\footnote{Answer accepted by the user who posted the question.} The majority of topics (81\%) have only one relevant document, and 17.5\% have two relevant documents. 
% To evaluate systems, mean average precision (MAP) is used. 


\textbf{NTCIR:} NTCIR-10, -11, and -12 used largely the same collections used for formula search tasks, consisting of arXiv papers and Wikipedia articles. The retrieval unit for NTCIR-10 was full documents, which makes assessment challenging. Therefore, in NTCIR-11, the retrieval unit was reduced to excerpts (roughly paragraphs), resulting in 8,301,578 search units. NTCIR-12 uses the same NTCIR-11 arXiv collection, and for Wikipedia pages, the retrieval unit is the full article.
These test collections contain different number of topics, growing in each lab. In NTCIR-10, there are 15 assessed formula+text topics. NTCIR-11 contains 50 topics, where each has at least one keyword and one formula. In NTCIR-12, topics were developed for search on two different collections: arXiv and Wikipedia. 29 arXiv and 30 Wikipedia topics were assessed. All the topics contained at least one formula, but 5 in the arXiv and 3 in the Wikipedia set had no keywords. 
All the NTCIR topics are lab-generated and only the query is provided with no additional description of information needs and search scenario.
Pooling methods also differ between the different collections \citep{evalarxiv}.

%For pooling, NTCIR-10 follows its formula search task approach, with each team submitting up to 100 documents per topic, and picking top-ranked documents until 100 documents are gathered for each topic. Each team in NTCIR-11 formula+text search task was allowed to submit up to 4 runs, returning the top-1000 results per query. For each topic, 50 retrieval units were chosen from the union of the retrieval results. In NTCIR-12, the top-20 ranked results per run were included in the pool for assessment.

The assessment process in NTCIR-10 for text+formula searches was similar to the formula search task, with the same assessors. The relevance was decided based on retrieved formulas, not documents due to size and complexity of documents in the collection.
%high number of formulas in documents, and having whole document as the retrieval unit.
For each formula, assessors used a graded 0-2 scale, to represent non-relevant (N), partially relevant (PR) or  relevant (R) judgements.
Each formula was assessed by one or two assessors. 

In NTCIR-11, assessors were shown the title of the topic, the relevance description, and an example hit (if any) as supplementary information. For this collection, relevance was determined using the roughly paragraph-sized retrieval units, rather than individual formulas. 
%That is to say, the assessors judged the relevance of each retrieval unit to the query based on the keywords, as well as the formulas included in the submission files. 
To make sure that assessors had enough mathematical background, they were chosen from undergraduate and students in mathematics for the arXiv topics, and computer science for the Wikipedia topics.
Relevance levels were the same as for NTCIR-11.
%, however, the assessors for Wikipedia topics were computer science students. 
Each hit was evaluated by two students, with their judgements combined. 
The final judgement was decided as R/R and R/PR as relevant (2), PR/PR, R/N, PR/N as partially-relevant (1), and N/N as not relevant (0). 

%The evaluation measures differed slightly across 
As for the evaluation measures, NTCIR-10 has MAP, P@\{5,10, hit\} as four basic measures. In NTCIR-11, in addition to MAP and P@\{5, 10\}, bpref was also included to handle unjudged instances. NTCIR-12 tasks reported P@\{5, 10, 15, 20\}. In all cases, relevance judgments for formula instances that were missing from the pools (as can happen for P@hit and MAP) were treated as not relevant.

\textbf{ARQMath:} ARQMath's main task is retrieving Math Stack Exchange (MSE) answer posts using MSE question containing formulas and text as queries. This was motivated primarily by three things: first, short answer posts are easier to assess (\ie usually at most a few paragraphs in a post, vs. complete papers), Second, a query log analysis \citep{mansouri_characterizing_2019} that showed that the number of question queries was almost 10\% higher for math searches compared to searches in general.  Third, the question posts act as both query and information need description.
%The task is defined as:
%\textit{Given a new mathematical question (not seen in training) find the relevant answers to it.}
ARMath's topics and collection are built from Math Stack Exchange, as shown in \reffig{fig:ARQMath}. All questions and their related answers posted from 2010 to 2018 are provided for training, including roughly 1 million questions and 28 million formulas. ARQMath topics are selected from the new questions posted in 2019, 2020, and 2021. 

\ourfigscaled
	{!t}
	{0.7}
	{figures/Evaluation/ARQMathMathSE}
	{ARQMath Answer Retrieval task built on Math Stack Exchange. Questions and their answers posted from 2010 to 2018 are available for training purposes. Topics are selected from new questions from 2019 on, and  answers are retrieved the collection of answers from 2010-2018.}
	{fig:ARQMath}

Overall, there are 226 assessed test topics: 77 in ARQMath-1, 71 in ARQMath-2, and 78 in ARQMath-3. 
A constraint for topic selection is that question posts should contain at least one formula, and 3 categorizations were assigned to candidate topics: 
\begin{compactenum}
\item \textbf{Topic type}: \textit{computation}, \textit{concept} or \textit{proof}
\item  \textbf{Difficulty}: \textit{low}, \textit{medium}, and \textit{high}
\item  \textbf{Representation dependency}: \textit{text}, \textit{formulas}, or \textit{both}
\end{compactenum}
%\reffig{fig:ARQMathTopics} shows counts of topics per category in ARQMath-1, -2 and -3.
These categorizations were used to diversify selected topics.  

The pooling process in ARQMath test collections are based on different cuts of participating teams. Each team was allowed to submit up to 5 runs, selecting one run as primary and the others as alternative. 
Deeper cuts were considered for primary runs. 
ARQMath provides all system runs used for pooling, which provides a way to study different approaches and understand their behavior in greater detail. 

ARQMath assessor for answer retrieval task were also selected from students in mathematics, similar to the formula search task. There were 2-3 training sessions with a math professor to introduce the task and train the assessors in each test collection. Some questions might offer clues as to the level of mathematical knowledge on the part of the person posing the question; others might not. To avoid the need for the assessor to guess about the level of mathematical knowledge available to the person interpreting the answer, we asked assessors to base their judgments on the degree of usefulness for an expert (modeled in this case as a math professor) who might then try to use that answer to help the person who had asked the original question. Four relevance degrees are considered for this task, defined in Table \ref{tab:ARQMathTask1Relevance}. All relevance ratings organized by topic and assessor may be found in a `big' qrels file available with the test collection.

Finally, for evaluation, the same evaluation measures as the formula search task were used: nDCG$^\prime$, MAP$^\prime$ and P$^\prime$@10. Prime metrics avoids issues discussed earlier for unevaluated hits when using test collections.

\ourtable
{!t}
{
% We need to use command Verb, not verb!! (Solved)
\begin{small}
{
\resizebox{\columnwidth}{!}{
\begin{tabular}{c l p{3.6in} }
\toprule
\sc Score~ & \sc Rating & \sc Definition\\
\midrule
3 & High & Sufficient to answer the complete question on its own \\

2 & Medium & Provides some path towards the solution. This path might come from clarifying the question, or identifying steps towards a solution \\

1 & Low & Provides information that could be useful for finding or interpreting an answer, or interpreting the question  \\

0 & Not Relevant & Provides no information pertinent to the question or its answers. A post that restates the question without providing any new information is considered non-relevant \\
\bottomrule
\end{tabular}
}
}
\end{small}
}
{Relevance assessment criteria for the ARQMath Answer Retrieval task.}
{tab:ARQMathTask1Relevance}

%To summarize, NTCIR and ARQMath test collections are commonly used for evaluating math-aware search systems. With the pilot task started at NTCIR-10, more and more was learned about developing math-aware test collections. For instance, starting in NTCIR-10, the retrieval units were the whole document, which made assessment hard, and that was reduced to paragraphs in NTCIR-11. With observation in NTCIR-11 and using Wikipedia as a simpler collection, NTCIR-12 used both arXiv and Wikipedia as the collection.

%NTCIR topics were all lab-generated. ARQMath, however, considered math questions posted by real-world users on Math Stack Exchange as topics. Topics were selected based on different categorizations to ensure diversity. ARQMath brought attention to prime effectiveness measure to handle unjudged answers which makes comparison fair for the future systems that did not participate in the pooling process. This approach can also be useful for pilot study of less efficient systems, and ranking the whole collection can be time-consuming. These systems can only re-ranked the assessed answers. 


%Table \ref{tab:mathaware-search-teams} summarizes the math-aware test collections, their collections, and the number of teams and runs participating in building them.





\textbf{Cross-lingual math information retrieval:} 
Current math search engines and test collections are primarily developed for the English language, limiting their accessibility and inclusivity. Cross-lingual math information retrieval (CLMIR) is a new task, focusing on retrieving mathematical information across languages. CLMIR has been explored for math-word problems \citep{tan-etal-2022-investigating}, where existing datasets were translated into Chinese using online machine translators, and manually refined the translations. CrossMath~\citep{gore2024crossmath} is a novel CLMIR test collection comprising manually translated topics in four languages (Croatian, Czech, Persian, and Spanish). These are the same topics used in the ARQMath Answer Retrieval task. This domain is fairly new and a research gap to be filled. There are approaches proposed for machine translation of mathematical text~\citep{9369381_1, petersen-etal-2023-neural} and more to come in the future.

\textbf{Other math-aware search collections:} With recent advances in conversational search, these models are explored for math as well. MathBot~\citep{grossman2019mathbot} is a text-based tutor capable of explaining math concepts providing practice questions and offering feedback to the students. Compared to other domains, there are no standard benchmarks developed for evaluating math conversational search systems. The use of clarifying questions for math has been studied on Math Stack Exchange by extracting comments on math questions~\citep{10.1145/3578337.3605123}. Tasks such as generating clarifying questions, and detecting ambiguous math queries can be studied on this dataset.   




\section{Searching with formulas and text} 
Math-aware search supports queries containing both text and math.
Unlike text or formula search where queries and sources have one representation, for math-aware search queries and sources combine text with  one or more formula representations (\eg SLT, OPT, or \LaTeX{} tokens). 
Because of the different representations (\ie \emph{modalities}), this is a math-specific variation of \emph{multimodal} information retrieval \citep{DBLP:journals/tkde/ZhuZGLYS24,DBLP:journals/mta/ShirahamaG16}.

A key challenge in multi-modal search is bridging the gap between diverse data formats like text, images, videos, and audio \citep{Bozzon2010}. 
There are two main approaches for searching multiple representations: searching modalities separately and combining rank scores to produce the final source ranking, or creating a unified representation for all modalities and searching this directly. 
Below is a summary of approaches that can be used to combine formula and text search for sparse or dense search indexes.

%Specifically for math-aware search, possible approaches to searching text and math include the following. 

% \rz{@Behrooz -- missing citation for which A0 version used in the previous sentence -- the 2023 model?}

\begin{compactdesc}
    \item  \textbf{Sparse retrieval:}\\Formulas are represented using text tokens (\eg in \LaTeX{}) or token sequences annotated on formulas after traversing nodes of formula trees (\eg depth-first traversal of OPT or SLT). These formula tokens may represent individual symbols, or tuples, \eg `+' node in OPT for $x+1$ as operator-prefix tuple $(+,x,1)$, or $(x, 1, \rightarrow \rightarrow)$ for the SLT path from x to 1.
    
    \begin{compactenum}
    \item \textbf{Independent:} text and each formula representation have their own inverted index. Query text and formula representations are separated before searches are run, and results are combined to score sources. 
    
    \item \textbf{Unified:} text and formula tokens belong to one vocabulary, and a `traditional' inverted index is used to search both together (see Ch. 1). Linearized formula tokens are inserted in source text before indexing, and text/math tokens produced for queries are looked up in the unified inverted index.
    \end{compactenum}
    
    \item \textbf{Dense retrieval:} \\
    Formulas and/or subexpressions representations are annotated with vectors in embedding spaces (see Ch. 2). Before embedding, formula representations may be linearized tokens (\eg \LaTeX{}), trees (\eg OPT, SLT) or other representations (\eg PHOC).
    
    \begin{compactitem}
    \item \textbf{Independent:} each text granularity (\eg token vs. sentence) and formula representation have separate embeddings.  Query text and formula vectors return the nearest-neighbor vectors in each space, with similarity scores combined to score sources.
    
    \item \textbf{Unified:} text and formula elements for sources and queries are embedded in the same dense vector space. Multiple space may be used for different granularity (\eg text+math in passages, vs. individual math/text token embeddings). Vector(s) for sources close to queries in the unified embedding space(s) are used to score sources.
    
    \end{compactitem}
\end{compactdesc}

%This can be done for math-aware searches by doing a separate formula and text search and combining the results. Another alternative is to unify the text and math representations and do one retrieval. 
Most systems that combine independent formula and text searches to date use sparse retrieval (\ie inverted indexes) to produce the initial retrieval results.
However some models combine sparse and dense retrieval models.
For example, ColBERT \citep{10.1145/3397271.3401075} has been used for text search, and the similarity scores linearly combined with formula search results produced using from Approach0, which was described in the previous chapter.

%As each of the approaches can have its benefits, ensemble models have been explored for math-aware search. 
As a concrete example of combining sparse and dense retrieval models, the MSM team at ARQMath-3 uses Reciprocal Rank Fusion (RRF) to combine  sparse TF-IDF and BM25 retrieval models with a %fine-tuned 
RoBERTa dense retrieval model.
The final rank score is produced by EQ.~\ref{eq:rrf} to combine retrieval results from a variety of systems, ranging from  In this equation, $R$ is a set of rankings, and $r(d)$ is the rank of document $d$. The proposed system achieved nearly the same nDCG$'$ value as the top system for the ARQMath-3 answer retrieval task (0.504 vs. 0.508).

\begin{equation} \label{eq:rrf}
RRF(d) = \sum_{r \in R}{\dfrac{1}{60 + r(d)}}
\end{equation}


We review the use of independent and unified text and math representations for search in more detail below. 
%In this section, we will review both approaches. 







\paragraph{Fusing independent formula and text search results.}
%\reffig{fig:fusedmathawaresearch} presents an overview of this approach.
With several sparse and dense formula search models available, one approach to math-aware search is combining text search with a separate formula search, and then combining the results. 
Techniques for combining the results include boolean constraints, linearly combining formula and text scores, learning-to-rank, and voting methods. 

\reffig{fig:fusedmathawaresearch} shows a math-aware search model that uses independent searches for text and formulas identify relevant sources (\eg documents or passages).
At indexing time, the \emph{extractor}  is used to separate the formulas and text of sources into two separate search indexes, and formulas are annotated with token sequences for sparse models, or embedding vectors for dense models.
At query time, the same extractor splits a query into sub-queries for text and formulas, and annotates formulas with a token sequence or vector.
%, and a separate formula search returns sources with formulas whose indexed patterns match based on indexed mathematical symbols or subexpressions. Finally, 
The results from both searches are combined into the final score for retrieved sources, and the final result is communicated to the user. 


\ourfigscaled
	{!t}
	{0.55}
	{figures/MathAwareSearch/FusedMathAwareSearch.pdf}
	{Fusing independent formula and text search results.}
	{fig:fusedmathawaresearch}
 
We'll next consider different approaches to fusing independent formula and text searches, starting with Boolean queries used to filter sources without both formula and text token matches.
MathWebSearch \citep{hambasan_mathwebsearch_2014} 
%uses OPTs (in Content MathML) and 
represents formulas as tokens for OPT subexpressions stored in a separate inverted index for formulas  (implemented in ElasticSearch).
%When a text+formula query is submitted, 
Both formula and text inverted indexes are queried separately. 
However, text search results are used only to implement Boolean queries of the form $(formula_1 \vee ... \vee formula_n) \wedge (term_1 \vee...\vee term_n)$, %where at least one formula token and one text token must be matched in each source. 
requiring at least one formula and one text token from the query to match a source.
Sources without text token matches are removed from the formula rank score list, which produces the final ranking.
%relevant formulas 
%run, and then a boolean filter is used to remove documents without a query text token match.
%The final score is computed by the best query formula match score -- the text tokens only serve to filter the results.  % ????
%using only the text tokens.
%Then, documents containing at least one of the query text tokens are selected. 
Despite the simplicity of this approach, the system achieved a $P@5$ of 0.79 for the NTCIR-11 math-aware search task (arXiv papers). 
% \rz{@Behrooz -- please check changes in the paragraph above; how scoring was done was not clear. What ranking function was used for the text tokens? And was I right about this being the arXiv data?

% ** Was I wrong about the representation for formulas here? I was trying to show the commonalitie/links between approaches in MathWS and MIaS, focused on the shared boolean query nature of the filters, but the description above may not be quite correct if Substitution Trees are used for search in MathWS.}

The same type of boolean query/constraint is used to combine formula and text results in the MIaS system \citep{sojka_indexing_2011}, %, where the input query is split into math and text parts. 
%uses separate sparse retrieval indexes for formulas and text implemented in Apache Lucene, using 
which uses canonicalized tuples as formula tokens (\eg with variable unification; implemented in Apache Lucene).
%Terms are appended to the formula search to create a boolean query with text terms as $(formula_1 \vee ... \vee formula_n) \wedge (term_1 \vee...\vee term_n)$. 
%Similar to MathWebSearch, only documents matching both a formula tuple and a text term are selected for ranking.
%This model was later used with Apache Lucene, where for a given text+formula query, 
%initial candidates with the same matching approach were used (match at least one term, and at least one formula from the query). 
Rank scores for sub-queries generated from different combinations of text and formula tokens are used to re-rank the remaining candidates multiple ways, and results from these rankings were interleaved in the final search result to improve the diversity of returned sources \citep{sojka_mias_2018}.

% \rz{@Behrooz, for MIaS were the rank scores from TF-IDF, BM25, or something else? The 'sub-queries' are standard sparse retrieval calls and scoring via Lucene, if I remember correctly.}


Simple averaging and linear combinations of rank scores have also been used. For the ARQMath Answer Retrieval task three baselines methods were used for answer retrieval:
\begin{compactenum}
\item Tangent-S formula search model (linearly combined OPT and SLT scores), 
\item TF-IDF text search model, and 
\item unweighted average of normalized ($[0,1]$) Tangent-S and TF-IDF scores.
\end{compactenum}
For Tangent-S, the largest formula (SLT) in the question's title was selected, and if no formula was used in the title, the largest formula in the question body was used. The combined model was more effective then the formula or text model in isolation.

Linearly combining (\ie scaling and adding) formula and text rank scores was used in the MathDowsers \citep{ng_dowsing_nodate} system, where Tangent-L results for formula search are combined with BM25$^+$ text search. For text search, a keyword extraction model was used to select tokens in question answer posts for use in text queries. 
MCAT \citep{kristianto_mcat_2016} also linearly combines formula and text rank scores, but for multiple formula (OPT, SLT) and  text indexes. 
Text is indexed separately at the paragraph and document (title, abstract, keywords, …) levels. 
%text region scores and formula similarity scores are combined using a linear combination. 
This model was the most effective for participating teams in the NTCIR-12, ArXiv math-aware search task, in part due to the rich variety of formula and text representations.

% \rz{Metrics fro combined T-S+TF-IDF model -- was this a large difference? Which year?

% Also -- did I interpret the Tangent-L + BM25+ combination correctly, and the query generation?

% **Am I right about the types of multiple indexes used in MCAT (this is only my recollection).}



%Another approach to combine the similarity measures of formulas and text is to use a boosting algorithm. 
The WikiMirs system \citep{gao2016math} uses a learning-to-rank approach to combining formula and text scores.
%The system tokenizes and indexes formula OPTs and text separately. 
OPT internal nodes for operations (including bracketing/grouping) are converted to sets of concrete and generalized terms (tokens). % (via unification). 
For example, the formula $(x+3) \times \frac{a}{b}$, is tokenized into 4 concrete terms, and four generalized terms with wildcards for argument subexpressions:
\begin{equation*}
\begin{array}{l l l l l}
 \mathbf{Concrete~terms:} & \{~ (x+3) \times \frac{a}{b}, & (x+3), &  \frac{a}{b}, & x+3 ~\} \\
 \mathbf{Generalized~terms:} & \{~ (*) \times *, 	& (*), 	& \frac{*}{*},   & *+* ~\}
 \end{array}
 \end{equation*}
 %and four generalized terms \{$(*) \times *$, $(*)$, $\frac{*}{*}$, $*+*$\}. 
 %After indexing the context and formula terms, the initial 
 At query time, query formulas are converted to tuples as shown above, and a set of candidate sources retrieved using inverted indexes for text and formula tokens. These candidates are then re-reanked using RankBoost \citep{freund2003efficient} applied to features focused on  formulas. This system achieved the highest P@K values among the participating teams in the NTCIR-12 Wikipedia math-aware search task. 
 
 % \rz{@Behrooz -- roughly what made the model effective? Also, this description does make clear how the final ranking is produced -- is the candidate selection the querying? I've made a change to the text above to try and capture what I think happens, which is inverted index retrieval of text and formula tuples, *followed by* rankboost re-ranking (LTR, this is a standard approach).}
 


% \rz{@Behrooz: please check my attempted clarification on how linear combination of text and math is (roughly) done for MCAT.}

The Borda Count has also been used to combine text and formula relevance scores. MaRec (Math answer Recommender)  \citep{10.1145/3624918.3625337} retrieves answers to math questions.
Answers in the collection are classified into topics using text-based Naive Bayes classification (\eg for algebra, geometry, etc.).
At query time all answers in the sub-collection for the question topic classification are ranked.
% based on the context and formulas in a candidate answer.  
%Answers are classified by topic in the 
%In the first step, the input query (math question) and answers (in the collection) are classified based on the topic (e.g., algebra, geometry, …) using a Multinomial Naive Bayes classifier. 
%This classifier is used to reduce the search space, considering the answers with the same subject as the query. 
%Queries are also classified, and only answers in the matching sub-collection topic are considered for ranking. 
Answer scoring is done using separate similarity measures for text and formulas. 
\begin{compactenum}
\item Text similarity: Kullback-Leibler (KL) divergence between question/answer token frequency distributions.
Token vocabulary used is chosen with Dirichlet Allocation (LDA \citep{DBLP:journals/jmlr/BleiNJ03}): terms that characterize topics are selected.\footnote{Entropy and cross-entropy are closely related to, and even derivable from KL-divergence.} 
% The vocabulary used for these token distributions is selected using Latent Dirichlet Allocation (LDA \citep{DBLP:journals/jmlr/BleiNJ03}) to identify terms that are discriminating between topics.
%used to measure the similarity of language models for question and answer, generated based on term frequency. 
%To consider important terms, this model integrates a word diversity measure in KL-divergence based on LDA trained on the math questions. 
%The role of LDA is to select terms that should be considered when measuring KL-divergence; those are the terms with high probabilities in LDA topics. 
\item Formula similarity: %uses the \textit{TreeMatch} model, which 
averages tree-edit distance on SLTs and a depth score, based on the sum of leaf-root OPT path lengths matching an answer.
\end{compactenum} 
The final ranking score uses the Borda Count, adding the number of answer posts that rank lower than a source in the formula and text rankings. 
% \textbf{???Effectiveness} -- given this was for ARQMath, how effective was the approach?

% \rz{@Behrooz, check my summary above, fix any errors. For example, I have assumed that all answer posts for a topic category are ranked, and that SLTs are used.

% In particular, not sure whether we classify for one topic, or some top-k topics, or something else.

% **Does depth score average the matched paths/branches? Are they just matching paths, and calling it something else? This sounds like an interesting variation of path matching + full tree structure ranking. Please check, revise as needed. 

% ***Effectiveness is missing; this is important. Is this method last because it is best-to-date? 
% }

% While using the full text for search is one approach, the alternative approach is to enrich math formulas with more relevant textual information. Instead of using fixed-size windows, the application of dependency graph has been explored \citep{kristianto_utilizing_2017}. 

% \rz{@Behrooz -- 



% there is a missing brief summary here. Is one combination approach generally more effective than another, or does this depend upon the effectiveness and combination of independent search indexes used? Something else?}


\paragraph{Unified representations for formulas and text.}
Combining results from separate indexes for different representations can often produce useful results quickly (especially using sparse retrieval models). However, the text-notation interactions described in Ch. 2 that provide important context for formulas is missing when formulas and text are represented separately. We next consider searching unified representations for formulas and text.
%Several approaches aim to propose a unified representation of math formulas along with text, and then, the traditional retrieval models are used for the search.

DLMF whose formula retrieval model is described in the previous chapter was the earliest unified sparse retrieval model indexed formula and text tokens together, using a variation of TF-IDF for scoring \citep{ miller_technical_nodate}.
More recently Latent Dirichlet Allocation (LDA) has been used to weight formula and text tokens. 
In these sparse models, formulas are represented as~\LaTeX~tokens \citep{yasunaga_topiceq_2019} or linearized tree tokens \citep{thanda_document_2016}, and a single inverted index is used to retrieve and score sources.


In the previous chapter, we saw formula dense retrieval models using the text context around formulas,
the majority of which embed text and formulas together using formulas represented by~\LaTeX~ tokens. 
The introduction of the ARQMath answer retrieval task coincided with the emergence of transformer-based models, and 
a common technique is using a pre-trained transformer (\eg BERT variants) that is fine-tuned using pairs of MathSE questions and answers with their associated assessor relevance ratings.

\paragraph{Using transformers with unified representations and math tokenization.} 
Reusch \citep{10.1007/978-3-031-13643-6_14} studied dense retrieval using ColBERT and ALBERT models. 
To fine-tune ALBERT, 1.9M triples containing questions with one relevant and one non-relevant answer were fed to the model. 
The model attempts to match assessor scores by classifying answers using the learned vector embedding for the \textit{[CLS]} token that starts each token sequence in an answer post. 
A similar approach was used to fine-tune ColBERT, but using more relevant and non-relevant answers. 
Somewhat surprisingly, both models proved less effective than sparse retrieval models that participated in the ARQMath-3 shared task. 
% \rz{@Behrooz -- guessing on how triples were scored (here, estimating the relevance of every individual relevant or non-relevant post -- but was this a binary classification task?
% I think I'm right about most embedding using LaTeX text/math data for embedding (that is far more prevalent, available data-wise), but let me know if I'm wrong there.

% **Moved discussion of transformers and reasoning to the section on QA/reasoning. This is out of place here.}
In subsequent work, the researchers explored how mathematical formulas affect a transfomer model's training \citep{10.1007/978-3-031-56027-9_15}. They found the transformer models consider formulas when scoring relevance for answers to a given math question. 
However, a study of the transformer attention weights for formula and text tokens suggests that structural relationships between formula tokens are lost, and that the attention maps do not consider variable overlaps between formulas appearing in questions and answers. This motivates creating transformer-based models that can better capture formula structure and interactions, which are relatively rare in sources used to pretrain transformers.
%better understanding of formulas.

% \rz{@Behrooz -- added 'do not consider' to description above, because looking at shared variables in questions and answers seems beneficial. I also assume this study was based on attention weights, please correct if I am wrong.}

One approach is adding additional tokens. The MathPredictor model \citep{jo-etal-2021-modeling-mathematical} extends BERT's tokenizers to support  2,651 new vocabularies. This addresses the BERT WordPiece tokenizer's oversegmention of \LaTeX{} commands such as `\textbackslash overline', which is split into three tokens: \{\textbackslash, over, \#\#line\}. This allows formulas such as $\overline h$ (in~\LaTeX~expressed as \verb|$\overline h$|) to be correctly tokenized as \{\$, \textbackslash overline, h , \$ \}. 
The model was then fine-tuned using masked tokens in formulas.
% \rz{@Behrooz -- replaced 2651 'new vocabularies' by 'new tokens'}

A similar approach is taken in the hybrid MABOWDOR system \citep{10.1145/3539618.3591746}, where the PyA0 toolkit is used for preprocessing mathematical formulas before tokenization by WordPiece. 
PyA0 canonicalizes math tokens by merging those likely to be semantically identical, such as \verb|\emptyset|, \verb|\empty|, \verb|\varnothing|. 1,000 new math tokens are added to the token vocabulary, and the math tokens are then treated similar to regular text. 
The final search used combines dense and sparse retrieval, and both independent and unified formula/text representations. 
A unified single-vector dense retriever is used for passage-level representations of formulas and text (DPR \citep{karpukhin-etal-2020-dense}),  math is searched independently using Approach0 (combining path-based sparse retrieval with structural alignment),  and a dense embedding-augmented sparse retriever (SPLADE \citep{splade}) is used to search text independently. 
% \rz{@Behrooz -- check notes above; some things may have been inferred incorrectly.}

For the MABOWDOR unified representation dense passage retriever, a new pre-training dataset for the math domain was created using the Coco-MAE retriever architecture and pretraining scheme. 
The pretraining task is Masked Auto-Encoding (MAE), which is similar to masked token pre-training but attempts to decode whole input passages with masked tokens using a decoder. For the final ranking, search results from each component are merged using a convex linear interpolation. This system currently archives the highest P$'$@10 for ARQMath's answer retrieval task.
% \rz{@Behrooz -- what is the decoder used for in Coco-MAE, rather than just predicting the hidden token? That is a form of decoder, so I'm unclear whether this is actually distinct from standard masked pre-training, just using data with text and formulas; is this trying to reconstruct an original sequence of \LaTeX and text tokens, for example? Please check.

% **Also -- does Coco-MAE have text and math token (as I assume...) or only math?

% **ALso -- is there any tradeoff between the P'@10 and the whole-ranking nDCG' and mAP' metrics? I mention this tendency in Ch 3. } 

In an alternative approach, MathBERT \citep{peng2021mathbert} (see previous chapter) uses linearized OPT tokens and~\LaTeX~formula representations.
BERT is pre-trained using Masked Language Modeling, Context Correspondence Prediction (similar to next sentence prediction), and Masked Substructure Prediction (for masked formula tokens). 
Using an improved tokenization approach for math formulas, this model archives better effectiveness compared to BERT in tasks such as formula topic generation (predicting the topic (tag) associated mathematical formula) (by creating  TopicMath-100K dataset on arXiv papers), and formula `headline' generation (EXEQ-300K \citep{Yuan_He_Jiang_Gao_Tang_Giles_2020}), creating a concise description of a formula using the formulas and descriptions in a MathSE question.

% \rz{@Behrooz -- are these tasks for MathBERT above done using ARQMath, or some other data source?}

Researchers then used MathBERT's language model for retrieval and other `downstream' tasks. For example, automatic math short-answer grading \citep{zhang2022automatic} by classifying grades using an integer ordinal scale from 0 to 4. The MathBERT model is fine-tuned for this task, with pairs of questions and student responses. Additional information such as the scale of the grade and example answer with grade is also passed to this model for in-context meta-learning. 

% \rz{
% **No mention of using MathBERT for retrieval, or the results for that --- +++please add, that's the focus of this section.

% **More broadly, MathBERT's connection to the main story re: transformers and tokens is unclear; please add -- where specifically were you trying to take the reader, in terms of the narrative/story? I can't see it here. 

% **What is the 'improved tokenization,' roughly? Is this just adding pre-defined tokens again?


% **Also assumed that the 'topics' are tags annotated on posts. Please correct and clarify if that is wrong.}

% \rz{@Behrooz -- moved RRF example for MSM to beginning where different ways to integrate math/text representations is summarized.}


%%%% Listing related work will put them back in order
% \citep{misutka_extending_nodate}


% \citep{ruuvzivcka2016math} 
% MIRMU \citep{liska_similarity_2013} uses Lucene, and pre-process math formulas by applying canonicalization and several generalization techniques. To allow searching of subformulae, expressions are tokenized and subtrees of formulae are extracted. After these steps, formula trees are linearized to reduce index space. 

\section{Using LLMs for math-aware search}


Despite the advances in LLMs, their capabilities for math information retrieval need further investigation. Some recent researchers aimed to explore this by comparing the results from LLMs against human-generated and assessed answers. 

The use of LLMs as both answer generators and re-rankers have been explored using ARQMath's answer retrieval task. Satpute et al. \citep{10.1145/3626772.3657945} considered both general LLMs like GPT-4 and math LLMs like ToRA to generate answers for ARQMath topics.  
These answers were then used as queries to search for relevant answers. 
This can help by transforming the query into a format more similar to sources in the collection, as the query and collection are expressed as answers. 
For each question, an embedding (using {\tt BERT\_cocomae}) of the generated answer was used to search dense embeddings for ARQMath answers, and cosine similarity was used to find the most similar answer to the generated answer. This approach is currently the state-of-the-art for ARQMath answer retrieval task, with nDCG$'$ of 0.486 (vs. 0.464 of BERT\_cocomae).

% \rz{@Behrooz, please check my revision of the last sentence above.
% You said this was effective -- is it SOTA? With what numbers?}

In another study, the applications of general LLMs, (LLaMA-2 and Orca-2) were studied for three tasks in math information retrieval: relevance assessment, data augmentation, and re-ranking (point-wise) \citep{10.1145/3626772.3657907}. This study was done on ARQMath dataset and for each task, an appropriate \textit{system message} is used; for example for assessing the relevance of an answer to a math question, the system prompt was created based on ARQMath assessment protocols as:
\begin{quote}
\it    You are a math professor who will assess the relevance of an answer to a given math question.
\end{quote}
The results of this study revealed that while general LLMs are not yet suited for relevance assessment or re-ranking, the data augmentation from Orca-2 which %has high reasoning capability can be as 
is useful for expanding the ARQMath training set for use in fine-tuning neural math answer retrieval systems. The data augmentation process is performed by generating additional relevant answers for each training topic using LLMs.

\section{Summary}

***TBD






==> figures/ch3-evaluation.tex <==
\chapter{Math Retrieval Tasks} % and Evaluation}
\label{c-eval} % a label for the chapter, to refer to it later






\section{Which tasks have been studied?}

In the math IR research community, ...

\ourfigscaled
	{!t}
	{0.25}
	{figures/Ch3-System-Overview}
	{Data and metrics from \reffig{fig:system} used for math retrieval and Q/A tasks. 
	  Test collections include a collection of sources, queries with information need descriptions (\ie \emph{topics}), query relevance assessments for individual sources returned in results (\ie \emph{qrels}), and effectiveness metrics. Q/A tasks return a single response compared to an ideal answer using a content-based effectiveness metric. }
	{fig:ch3overview}

In this chapter, we consider the specific test collections and evaluation protocols that have been used to evaluate mathematical information retrieval systems.  As part of this, we describe the retrieval tasks that have been used to compare retrieval models, including their source collections, inputs, outputs, and evaluation metrics.

TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBDTBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD 

TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD TBD 

\input{ch3-task-examples}

% +Efficiency metrics/evaluation mention/notes



%%%%%%%%%%%%%%%%%%%%%%%%%%%
% EVALUATION
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Evaluating retrieval}

\begin{myexample}{Evaluating Retrieval Systems}{eg:eval}

\section*{Standard IR evaluation framework}
\centering	
	\scalebox{0.45}{\includegraphics{figures/Evaluation/BehroozEvalFigure}}

~\\

\flushleft
\section*{Creating query relevance judgement files (QRELS)}
\centering
	\scalebox{0.45}{\includegraphics{figures/Evaluation/SharedTask.pdf}}

\end{myexample}

%:TEST COLLECTION CREATION
\section{Creating test collections}

Standard test collections provide a controlled environment with a well-defined set of documents and pre-judged relevance for each query. This allows for a fair comparison of different information retrieval systems without external factors influencing the results. One common approach for building test collection is through shared tasks. Conferences and forums such as TREC (Text REtrieval Conference), CLEF (Conference and Labs of the Evaluation Forum) and NTCIR (NII Testbeds and Community for Information access Research) provide a platform for 
shared tasks and building standard test collections. Each initiative defines a set of tasks and provides participants with access to a document collection and topics. 

Evaluating information retrieval systems relies on creating search scenarios that mirror real-world user experiences. We achieve this through topics, which represent a user's information need. A topic acts as a two-part key. The first part is the information need, a natural language description of what the user is looking for. This description provides context and clarifies the user's intent behind the search query, which is important for assessments. The second part is the query, which is the specific question or keywords a user might enter into a search engine.

As the goal of (offline) evaluation is to study how well a system will work in the real world, it is better to have a set of topics that are from real-world users. These topics can be from query logs or community question-answering websites. On the other hand, lab-generated topics can be useful when aiming to explore specific scenarios for new features. 

Topics and collections are provided for the participants who would develop and submit their runs. Each run consists of a ranked list of documents that the system retrieves in response to each topic. Then a pooling process is applied to select a set of candidate documents for assessment. Assessing relevance in math information retrieval is inherently challenging. This task needs assessors with strong mathematical backgrounds. Even with having strong mathematical backgrounds, assessors should be trained for assessment tasks; they should be provided with well-defined relevance definitions, and instructions to distinguish between different relevance degrees. A user's mathematical expertise can influence their perception of relevance. A highly technical document relevant to a math expert might be irrelevant to someone with a basic understanding of math. 

Assessment in math information retrieval can be challenging, due to the hard nature of distinguishing relevant documents, and their relevance degree. Assessor should be trained properly for the related tasks. During the assessment, usually, measures of agreements between assessors are reported. This is done by providing the same set of topics among assessors and comparing their assessments with agreement measures such as Cohen's Kappa coefficient. Properly training assessors can help increasing agreement among assessors. For instance, in ARQMath-3 \citep{mansouri2022overview}, for the formula search task, the Cohen's Kappa value increased from 0.21 to 0.52 from the first training to the last (third) training sessions. Another challenge, is to correctly assess relevance, the assessors might need to spend more time understanding the candidate document. In ARQMath test collection, for formula search task the average assessment time was around 35 seconds for each pair of formula query and candidate formula. For the other task, finding answers to math questions, which is a more complicated task, assessment time was approximately 64 seconds for each candidate answer.

Once the assessments are done, evaluation protocols are needed before measuring effectiveness. Consider a scenario from the previous example in Table \ref{tab:eresults}, where a system retrieves different instances of formula $y=\frac{a+bx}{c+x}$ from different posts as its top results, while its later results are not relevant. Should this system be considered as an effective model? For reasons like this, test collection like ARQMath (see the next sections) introduced an evaluation protocol for considering visually distinct formulae for evaluation. After applying evaluation protocols, systems are compared through a set of effectiveness measures. 
 
In information retrieval, creating evaluation protocols happens through several cycles and years of effort. Math information retrieval was no exception. 

\begin{myexample}{Contextualized Formula Search Assessment (ARQMath)}{eg:turkle}
	\scalebox{0.62}{\includegraphics{figures/Evaluation/Turkle3}}
	The Turkle assessment interface for the ARQMath Formula Search task is shown above. Left: the formula query is highlighted. Right: two question posts containing the same formula are shown. Assessors consider context by checking the question a query appears in, and the answers that retrieved formulas appear in.
\end{myexample}

%: RELEVANCE
\paragraph{Relevance Definitions and Assessment.} For effectiveness measures such as \emph{recall}, \emph{precision}, or mean reciprocal rank (\emph{mrr}) to be informative and useful for design and research, how relevance is defined and identified for a test collection is important. Most commonly a \emph{qrels} (quantitative relevance assessments) file is used to record which documents in a test collection are relevant for each test \emph{topic} in the collection.\footnote{The most standard qrels format was defined for the TREC conference series (\url{https://trec.nist.gov/data/qrels_eng})}
Sources in a qrels file have normally been evaluated by one or more human \emph{assessors}, using either \emph{binary} relevance (indicated by 0/1, with `1' for relevant) or \emph{graded} relevance on an ordinal scale (\eg for `non-relevant,' `low', `medium', and `high' relevance, identified by the integers 0-3). 




%% RATINGS example
\begin{myexample}{Relevance Assessments}{eg:ratings}
\scriptsize

\section*{Binary relevance and \emph{unknown} (?) relevance in results }

\centering
    \begin{tabular}{ c| l  c |  l c}
        \toprule
            & \multicolumn{2}{c |}{Model A}  & \multicolumn{2}{c}{Model B}\\
            Rank & Formula & Relevance & Formula & Relevance\\
            \midrule
            1 & $y=\frac{a+bx}{c+x}$ 	& \textbf{1}			& $g(x)=\frac{x}{x-a}$ 	& 0\\
            2 & $y=a+bx$ 			& 0			& $y=\frac{a+bx}{c+x}$ 	& \textbf{1}\\
            3 & $y=\frac{a-bx}{c-x}$ 	& \textbf{?} 	& $y=\frac{a+bx}{x+c}$ 	& \textbf{1}\\
            4 & $y=\frac{a+bx}{x+c}$ 	& \textbf{1}		 	& $y=\frac{a+x}{b+cx}$ 	& \textbf{1}\\
            5 & $g(x)=\frac{x}{x-a}$ 		& 0			& $y=a+bx$ 			& 0 \\   
      \bottomrule
    \end{tabular}

~\\
~\\

\flushleft
\section*{Graded relevance (0-3: Non-Relevant, Low, Medium, High)}
\centering

\begin{tabular}{p{1.25in} | c p{1.25in} | l }
       %\toprule
            \textbf{Query} & \multicolumn{2}{l}{\textbf{Result}} & \textbf{Relevance}\\ %Rank & Formula \\
            \hline
    


%{\sc Formula Query inside a Math Question(Topic B.4)} 


I have the sum 
%\mbox{~~~~~~~~~~~~~~~~} 
%\linebreak
%\fbox{
$$\sum_{k=0}^{n} {n\choose k} k$$
%}
know the result is $n^2-1$ but I don't know how you get there. How does one even begin to simplify a sum like this that has binomial coefficients.
&

1

& 

\vdots  
which can be obtained by manipulating the second derivative of 
$$
 \sum_{k=0}^n {n\choose k} z^k
$$
and let $z = p/(1-p)$
\linebreak
\vdots

&

\textbf{(3) High relevance}
\\

%\hline
&

2

&
%{\sc Non-Relevant}
Yes, it is in fact possible to sum this. The answer is 
$$
\sum_{k=0}^n{n\choose k}{m\choose k}={m+n\choose n}
$$
assuming that $n\leq m$. This comes from the fact that 
\linebreak
\vdots

&
\textbf{(0) Non-relevant}
\\

\bottomrule
\end{tabular}

\end{myexample}

A topic corresponds to a query accompanied by additional information for identifying relevant documents. Specific topic elements differ across test collections, but a topic normally provides (1) a description of an information need, (2) a query used for search, and  (3) a description of criteria and procedures for identifying relevant sources. 

In Chapter \ref{c-sources}, we discussed the ambiguities, context-dependence, and complexity of language, and in particular mathematical texts that include formulas, whose correct interpretation may require some amount of mathematical expertise.      The reader may note that in deciding which documents are relevant to a query using a topic description, what will be stored in a qrels file is influenced by both the interpretation of the person who wrote the topic description and the interpretation of the topic description by assessors scoring sources. [?? Ways around]

But how do we select the documents to be scored and stored in a qrels file, particularly for a very large collection? In the early days of IR research, the Crandall evaluations actually performed \emph{exhaustive} evaluation of all documents in a collection for a set of search topics. [...] Later it was determined that meaningful differences between models could be found using much smaller samples of documents in a collection. 

%: Pooling, assessment, experiments
\paragraph{Pooling, Assessment, and Experimentation.}
In a \emph{pooling} approach to sampling documents for evaluation,
sources are returned by `runs' (results) from a group of retrieval systems, possibly along with `manual runs' that are search results modified by, or even generated by people (these are often used to increase the number of relevant documents in qrels files). Most commonly pooling is performed by selecting the top-k (\eg top-20 or top-50) results from each system, and then identifying the set of \emph{unique} sources in these top-k results for use in assessment. In our experience, the depth of the pools (\ie values of $k$) used are determined by practical concerns, particularly the available budget for assessor time and compensation.

Earlier we had an example where we were measuring \emph{recall@10} using a qrels file, and obtained an average \emph{recall@10} of 50\%: on average half of the relevant sources in a collection were returned for each query/topic. This immediately suggests some important questions: 
\begin{enumerate}
\item What is the effect of missing relevant sources in the qrels file?
\item What is the effect of incorrect relevance assessments in the qrels file?
\item Are assessor grades/annotations in the qrels file consistent? 
\end{enumerate}

For the first question, missing relevant documents in the qrels file may be ignored while computing effectiveness metrics, or even penalized by being treated as non-relevant.\footnote{This is the default for many metrics in the widely used {\tt trec\_eval} tool, \eg for \emph{precision@k}}  For the second question, incorrect assessments may lead to undesirable decreases or increases in effectiveness metrics; whether these differences are concerning depends upon their frequency and character (\eg one query with many errors may be less concerning than multiple queries with errors of the same type). 

For the third question, assessors with low agreement may result in unclear or even contradictory results across queries, or within results for one query. Often task organizers will compute correlation coefficients between assessors for to quantify agreement, for example using a kappa correlation. Generally speaking, the larger the number of assessors, and the more unclear or complex the assessment task, the less highly correlated the assessor responses will be due to disagreements in judgement, differing interpretations of assessment criteria, and user errors caused by the required mental effort to evaluate (\eg clicking the wrong relevance score button). 

And so, we see that many variables influence effectiveness metrics computed from a qrels file: the chosen topics, the topic designer(s), the assessor(s), and the pooling method used to sample sources for assessment, along with other factors such as the assessment interface, and choice of relevance scores. For large collections with many topics, missed relevant documents and uncertainty/errors in relevance assessments are essentially unavoidable -- people make mistakes, and there is not time or even the energy needed to manually examine every collection source for every topic. 

Before we despair, note that our lack of `perfect answers' for test collections is true of all supervised pattern recognition and machine learning tasks.  
Fundamentally, machine learning algorithms with any form of supervision can be understood as playing \emph{imitation games} scored against the target outputs, generated by people: 
this is true whether people define targets explicitly (\eg relevance assessments), or indirectly in the use of human language for `self-supervision' (\eg in predicting the next word in a sentence, or next symbol in a formula).\footnote{Alan Turing's imitation game, an experiment designed to identify machines perceived as `intelligent' uses a sample of persons who interact over teletype with a computer and machine depends upon target values: whether a human participant selects the machine or person as the other human participant in the experiment). \missing{Turing 1950}} 
Some form of `target' values for labels, ranks, or scores are used for evaluation and in loss metrics. 
So what might seem to be a crisis of imperfect and incomplete relevance assessments is in fact a common limitation of the scientific method in general, and in the social sciences in particular where \emph{people} are under study. 
Effective retrieval depends upon our ability to create sources desired by people when performing search tasks, but where people, their preferences, and their behaviors vary tremendously and for myriad  reasons.\footnote{This interaction with the diversity of humanity is challenging, but also a very humanistic and beautiful aspect of IR research.}

This raises an important related point about scientific conclusions in general. Because of limitations in available data, and the limitations of experimentation itself, all experimental observations and outcome should be considered as \emph{evidence} for hypotheses, and never \emph{proof}. Proof requires that a hypothesis can be shown to be valid or invalid for \emph{every} possible input to a model or system: for example, the Pythagorean theorem can be shown to hold for every possible integer, and so we can construct a \emph{proof} that it is universally true for the set of integers. In contrast, an experiment on mathematical question answering will use a test collection with a finite number of test queries (miniscule in size compared to the set of countably infinite integers), and so results from an experiment using this collection observes a \emph{sample} (portion) of the space of possible queries and associated relevance assessments. In a sense, a proof tests a property for all possibilities of interest (\eg $\forall x \in X, \textrm{property}(x)$), while experiments  test properties  for some possibilities of interest (\eg $\exists x \in X, \textrm{property}(x)$). And this is true for mathematics, chemistry, physics, psychology, and information retrieval.

Thus, provided that we understand well-designed test collections as providing observations for use in collecting evidence in experiments, we needn't be overly concerned if in other settings/collections the same result is seen, provided that we then carefully study the potential reasons for their differences, and how they relate to the original assumptions used to design these experiments.

Related to our information task model in \reffig{fig:placeMatTasks}, experimentation is a valuable form of \emph{applying} information from available sources to \emph{create} new information sources such as research papers.\footnote{Galileo expressed concern about those who primarily consulted book indexes rather than carried out experiments in the real world, see \citep{duncan} pp. 9-10.}
Creating a test collection involves creating an information source that may be used for a variety of experiments.
However, running a useful experiment requires careful checking at each stage, including creating hypotheses and experimental designs, execution steps, and analysis and reporting. Fundamentally the scientific method's strengths and challenges come from its dependence on assumed information (\eg for making predictions in hypotheses) and its reliance on sampling possible inputs and reported observations. 

More concretely, experimental observations may be vague or incorrect for a variety of reasons, including:
\begin{itemize}
\item experiment designs that measure the wrong variables, or ignore important variables that affect the outcome (\ie confounds), 
\item issues with data sources used, such as sample bias or an insufficient number of observations (\ie `not enough data'),
\item imprecise or inaccurate measurements, and/or incorrect reading and reporting of measurement values, and
\item incorrect execution (\eg from bugs or using incorrect input files).
\end{itemize}
These are important possibilities to keep in mind both when interpreting reported experimental results and when running experiments of our own.

While experiments provide evidence and not proof, and almost no actual experiment is entirely error free, experiments providing reliable information, insights, or confirmation/contradiction of prior results are valuable additions to our available information sources. Experimental sources such as research papers are most useful when we read them skeptically (\ie question) as we consider their experimental designs, execution, and results.  At its best, experimentation aims primarily to inform and provide insight (\eg this is why/when retrieval model X outperforms model Y)  rather than impress (\eg `state-of-the-art results' without analysis of their cause(s)).

To avoid biases in model comparisons, even in cases of disputed relevance assessments in a standard collection, we normally report performance measures using the provided qrels file. 'Cleaning up' a qrels file by adding or revising entries is normally to be avoided, as it prevents direct comparison with other published work using the collection: this changes the `correct answers.' That said, it is not uncommon for authors to note in a paper when they find issues with or disagree with provided qrel data.


\section{Evaluation metrics}

Information retrieval systems are like the librarians who search through massive amounts of data to answer information needs. But how do we know if they are doing a good job? Consider top-5 retrieval results from two formula search models in Table \ref{tab:eresults}. Which system would you prefer?

As you might have guessed, one might prefer model `A' as its first result is relevant, while another may prefer model `B' where more relevant formulae are retrieved. Unjudged formulae are another issue; one way is to consider them non-relevant, while the alternative approach is to ignore them and move to the next judged document. Therefore, we need standard effectiveness measures to compare the systems. Figure \ref{fig:evalFlowchart} shows a high-level view of evaluation information retrieval systems.


\ourtable
	{!t}
	{

		\scalebox{0.625}{
		\begin{tabular}{p{0.75in}      p{1.5in}  l  p{2.25in}}
		\toprule
		 & \bf Name & \bf Formula & \bf Description \\
		%\hline 
		
		~\\
		\multicolumn{4}{l}{\bf Binary Relevance}\\
		\midrule
		RR 	& \textbf{Reciprocal Rank}			 
			& $1/k_f$ 
			& \mbox{Inverse of rank  $k_f$ for the} \linebreak first  relevant source 	 \\
		mRR & Mean Reciprocal Rank 		 
			& $\displaystyle \frac{1}{|Q|}\sum_{q \in Q} RR(q) $ 
			&  Avg. RR for query set $Q$ 			\\
		
		\hline
		R \emph{or} R@hit & \textbf{Recall}
			& $|S \cap R| / |R|$
			& Percentage of relevant in returned \\
			
		R@k & Recall at (rank) $k$
			& $|S_k \cap R| / |R|$
			& \mbox{Percentage of relevant in first $k$} \linebreak sources returned \\
		\hline
			
		P \emph{or} P@hit & \textbf{Precision}  
			& $|S \cap R| / |S|$		
			& Percentage of returned in relevant\\
			
		P@k & Precision at (rank) $k$
			& $|S_k \cap R| / k$	
			& Percentage of first k returned in relevant set\\

		
		AP	& Average precision			 
			& $\displaystyle \frac{1}{|R|}\sum_{k \in K_r} P@k(S_k)$  
			& Avg. $P@k$ for relevant documents appearing at ranks $K_r$ in $S$\\
			   
		
		mAP & \mbox{Mean Average Precision} 	
			& $\displaystyle \frac{1}{|Q|} \sum_{q \in Q} AP(q)$ 
			& Avg. AP for query set $Q$\\

		

		%\hline
		~\\
		\multicolumn{4}{l}{\bf Graded Relevance}\\
		\midrule	
		DCG@k & \textbf{Discounted \linebreak \mbox{Cumulative Gain}}
			& $\displaystyle r_1 + \sum_{i=2}^{k} \frac{r_i}{\log_2 i}$ 
			& Sums relevance scores $r_1$ through $r_k$ for returned sources $S_k$ using $\log$ discount from rank 3 on\\
		iDCG@k & \emph{Ideal} DCG   
			& 
			& DCG@k for reverse sorted grades of relevant sources $R$, \eg ($r_1, \ldots, r_5) = (3, 3, 2, 1, 0)$\\
		nDCG@k & \mbox{Normalized DCG} \linebreak \mbox{at (rank)} $k$ 
			& $DCG@k / iDCG@k$
			& Percentage of ideal DCG obtained for returned sources $S_k$\\
		\mbox{nDCG or} nDCG@hit& Normalized DCG
			& $nDCG@k ~\textrm{for}~k = |S|$
			& nDCG for all returned sources $S$\\

		
		~\\
		~\\
		\multicolumn{4}{l}{\bf Scored Sources Only: Includes Non-Relevant Sources $N$ }\\
		\midrule

		
		Bpref & \mbox{\textbf{Binary preference}} \linebreak \emph{(w. binary relevance)} 		
			%& $\displaystyle \frac{1}{|R|} \sum_{k \in K_r} \left(1 - \frac{ \min( |S_k' - R|, |R| )}{|R|} \right) $ 
			& $\displaystyle \frac{1}{|R|} \sum_{k \in K_r} \left(1 - \frac{ \min( |S_k \cap N|, |R| )}{|R|} \right) $ 
			&  Avg. percentage relevant before non-relevant for relevant sources; treats $|N| = |R|$ to balance classes. \\
			
		M$'$ & \mbox{\textbf{Prime metric}} (\eg P$'$@5, nDCG$'$)  	
			& \emph{(as defined for metric $M$)} 
			& Compute $M$ with $S' = S \cap(R \cup N)$ rather than full ranking $S$ \\
		
		\bottomrule
		\end{tabular}
		
		}
	
	}
	{Metrics for Search. By default, returned sources not in relevant source set $R$ are considered non-relevant. 
	$S_k$: first $k$ sources returned. \textbf{Note:} reported metrics are typically \emph{averaged} over queries but only mAP and mRR explicitly. 		Ch. 8 of Croft et. al's textbook provides a helpful overview of these metrics \citep{DBLP:books/daglib/0022709}. 
	%Prime metrics change this by ignoring sources in $S$ without a relevance rating.
	}
	{tab:smetrics}



%:%%%%%%%%%%% TURKLE %%%%%%%%%%%%%%
%\begin{myexample}{Contextualized Formula Search Assessment (ARQMath)}{eg:turkle}
%	\scalebox{0.62}{\includegraphics{figures/Evaluation/Turkle3}}
%	
%\paragraph{Relevant assessment.}	The Turkle assessment interface for the ARQMath Formula Search task is shown above. Left: the formula query is highlighted. Right: two question posts containing the same formula are shown. Assessors consider context by checking the question a query appears in, and the answers that retrieved formulas appear in.
%\end{myexample}

In information retrieval, when searching a collection of sources we distinguish two main performance measure types based on returned sources, and system behaviors. These correspond to (1) \emph{effectiveness} and (2) \emph{efficiency} measures. Generally speaking, effectiveness measures characterize search results by their coverage of relevant sources for user queries (\eg $recall$), and the rank position(s) of relevant sources returned (\eg $precision$).  
For retrieval tasks where the diversity of returned sources is important for users, additional measures are used [EXAMPLE?]. The primary efficiency measure for users is the query latency, for example, as measured by Mean Response Time ($mrt$).\footnote{\ie we don't like to wait.} 

% REVISIT in Ch 4.
Properties of search results for collections of sources  -- themselves an important structured \emph{source} that users frequently consult for information -- tend not to be studied in most evaluations of text-based retrieval systems. However, they were \emph{heavily} studied in the early days of internet use by the general public, and standard design principles have emerged \missing{Marti, others...}. For example, users generally expect to see matched query terms shown in bold, and in-context within document excerpts. 

For search results that introduce new modalities, \eg formulas in math-aware search, the effect of Search Engine Result Page (SERP) presentation on user effort and search effectiveness are important, and can be studied using in-lab, test-collection, and search log-based methods (\eg by observing time needed to find relevant items, questionnaires, user behaviors from screen capturing tools or longitudinal studies, etc.). For MathIR this remains an important issue that we will revisit in the next chapter.

For IR system designers and researchers, in addition to satisfying user goals effectively and efficiently,  there are additional performance measures that impact design decisions. These include indexing time, index size (on-disk and/or in-memory), query throughput (\eg queries processed per second), and measures for efficiency and effectiveness of algorithms used to annotate sources in the search index (\eg extracting formulas from PDF). 
These additional measures have implications for both hardware requirements and the quality of results that can be returned to a user quickly. 

In terms of \emph{information}, there is an important trade-off between retrieval time, index size, and search result quality.\footnote{related to the engineering adage `Fast, good, or cheap? Pick two.'}
The time-space efficiency tradeoff for algorithms is well understood: the more information that we have stored, the less we have to compute when running an algorithm. 
However, if we assume that the \emph{quality} of a search engine is measured by retrieval effectiveness, there may be additional source annotations that can be added to an index to increase effectiveness (\eg word or formula locations), or computed at retrieval time (\eg additional similarity scores used for reranking). 
%In this way, improving effectiveness may require additional information whose computation decreases space and/or time efficiency: 
Put briefly, the more source annotations that a system requires to be \emph{effective} and produce high quality search results, the less time and/or space \emph{efficient} the system will be, because the  amount of generated data has increased.\footnote{This assumes correct and optimal algorithm implementations. In practice, debugging and algorithm refinements also improve effectiveness and efficiency. } 
The additional annotations must be stored, computed, or some combination of the two, leading to a time / space / effectiveness tradeoff.

In some interesting cases, it is possible to improve both the efficiency \emph{and} effectiveness of a retrieval system. 
This happens when we identify a different retrieval model that uses `better information' for ranking, in the sense of being simpler and more compact (\ie requiring fewer annotations) while improving search result quality. 
For example, in the early days of information retrieval, some believed that detailed language models with formal grammars were important for retrieval. Such a model might require constructing a parse tree for every sentence in a collection, which must be stored and then searched at retrieval time. 
However, models based primarily on word counts and positions outperformed these more complex models \missing{I think Crandall demonstrated this: key researcher?}, while requiring much less computation at indexing and retrieval time (\ie less space and time). \emph{BM25} remains an important state-of-the-art technique based on term frequency, and owes its effectiveness and speed to using simple patterns for matching (\ie words) and a carefully considered and inexpensive ranking function producing high quality ranking.  

\ourtable
	{!t}
	{	
		\scalebox{0.7}{
		\begin{tabular}{l      p{1.5in}  l  p{2.25in}}
			\toprule
			\bf & \bf Name / E & \bf Formula & \bf Description \\
		~\\
		\multicolumn{4}{l}{\bf Correctness and Uncertainty}\\
		\midrule		
		EM & Exact match 
			& $\displaystyle \frac{1}{|Q|} \sum_{k \in Q} \delta(s_k, q_k)$
			& Percentage of answers identical to target answers ($\delta$ returns 0/1)\\
			
		Accuracy & Response accuracy 
			& $\displaystyle \frac{1}{|Q|} \sum_{k \in Q} e(s_k, q_k)$
			& Percentage correct answers w. tolerances in function $e$ (returns 0/1) for questions $Q$\\
			

			
		Perplexity & Average perplexity of selecting an alternative
			& $\exp(\ell_{CE}(S) / |Q|)$
			& Uncertainty for correct answers: no. equally likely alternatives = avg. cross-entropy loss. \\
			
		~\\
		\multicolumn{4}{l}{\bf Similarity to Text Answers (including Rationales, Step-by-Step) }\\
		\midrule
		Edit distance & String edit distance 
			&
			&\\
		
		Token F1 & 
			&
			& \\
			
		BLEU & 
			&
			& \\
			
		sBLEU &
			&
			& \\
			
		BERTScore & 
			&
			& \\		
				
		\bottomrule
		\end{tabular}
		}
		
		\scriptsize
		~\\		
		\linebreak
		$\delta(a,b) = (a=b)$; $e(a,b) = (normalize(a) = normalize(b))$; $\exp(x) = e^x$
		
	}
	{Metrics for Question Answers. For automated evaluation, metrics are computed from one or more selected `valid' answers. Here the queries $Q$ are questions expecting answers of different types. The answers are given in responses (\ie sources $S$).  }
	{tab:ametrics}

As seen in \reffig{fig:system}, a key decision for a search engine designer then, is which annotated information to include in the index, and how to search indexed annotations at run-time. 
As system designers, we particularly want to avoid (1) components that decrease efficiency without substantially improving or actually \emph{harming} effectiveness, and (2) potential increases in efficiency or effectiveness that are prohibitively expensive to implement. 
Researchers aim to assist designers through identifying new ways to improve effectiveness and efficiency in retrieval models, and to formalize and strengthen our understanding of retrieval processes both in part and as a whole (\eg through studying users and proposing new, informative performance measures). Researchers also encounter their own design decisions when creating systems for experimentation.

The experiences of system designers and findings of researchers are mutually reinforcing: researchers propose new analysis techniques and retrieval models that designers may use, who in turn report on how they are found to work in practice, and at scale with large numbers of users. Effectiveness and efficiency measures are a key part of this interaction, identifying areas of strength and potential improvement in models and implemented systems. 

\paragraph{Comparing Performance Metrics.}
Whether a difference between models or systems is `substantial' is important for both researchers and designers. As just mentioned, designers prefer to avoid computing or storing additional information that does not improve effectiveness meaningfully (\eg a consistent `noticeable' improvement), and researchers will want to know whether observed differences are likely to be consistent for queries not seen in their experiments.  

Most retrieval performance metrics are reported as averages over queries. For example, when we talk about the \emph{recall} of a system, we are normally referring to the \emph{average recall} obtained over all queries tested, and similarly for \emph{precision}, $MAP$, $MRR$, $nDCG$, etc.
While it is tempting to compare using only these performance measures averaged  over queries, the \emph{variance} in the values used to compute the average is important. 

As a simple example, imagine that we have two retrieval systems that return exactly 10 results for each query. In an evaluation, we observer that both systems have an average \emph{recall@10} of 50\%, as computed using a \emph{test collection} consisting of math question and answer posts, a set of question queries, and a \emph{qrels} (quantiative relevance assessments) file identifying relevant answer posts for each question query.  In one system, 50\% of the relevant documents in the \emph{qrels} file are always returned. In the other, half of the query questions return \emph{no} relevant answers from the qrels file (\ie $recall@10$ of 0\%) while the other half return \emph{all} relevant answers in the qrels file (\ie \emph{recall@10} of 100\%). 

In this artificial example, the first system has no variance in \emph{recall@10} values at all: the performance is identical for all queries. In sharp contrast, the second system oscillates seemingly randomly between perfectly relevant and perfectly awful results. So while both systems have an average \emph{recall@10} or 50\%, one system is consistent, while the other returns no relevant sources half of the time. In this example, despite having identical average recall values, the difference in the \emph{variance} of recall values for individual queries are clearly different. Further, it suggests we would probably prefer to use the first system, because it is more consistent and avoids missing relevant answers altogether.

Particularly for formal experiments, we want to compare \emph{distributions} (\ie sets) of performance metric values rather than averaged metrics in isolation.
In information retrieval, statistical hypothesis tests are used to estimate whether differences in average measures are likely to continue being different over additional queries. They include an estimate for  a Type-1 error (\ie the \emph{p-value} for false detection of a difference where none exists). Generally we consider a \emph{p-value} less than either 5\% or 1\% (\ie $p < 0.05$ or $p < 0.01$, chosen \emph{before} running an experiment)  to be a `statistically significant' difference indicating that it is \emph{expected} that distributions will continue to differ for additional queries. These estimates of how likely two distributions remain distinct with more observations is possible because of assumptions about distributions (\eg a common assumption for \emph{parametric} tests is normality/Gaussian shape), and these assumptions differ between statistical hypothesis tests.\footnote{In technical papers the phrase `significant difference' should only be used when a statistical hypothesis has been used.}

Commonly used statistical hypothesis tests for performance metrics averaged over queries include the standard t-test for comparing two distributions, and the Bonferonni \emph{corrected} t-test when comparing average measures for two or more other models to a baseline system. Many other tests and comparison types (\eg using correlation coefficients, and Wilcoxin rank sum tests to compare ranked lists) are used in IR, but this is not a focus of this book, and we direct the reader elsewhere for details.\footnote{we briefly note that \emph{effect size} is another important issue in rigorous statistical comparisons. For example, a significant but very small effectiveness improvement may not be meaningful for a real-world system, particularly when considering efficiency costs and/or implementation effort.}

Finally, when comparing performance metrics, for designers and researchers it is \emph{critical} to note  the \emph{specific} queries where performance differs substantially, \ie where a query obtains notably higher/lower measures. While measures averaged over queries can identify broad trends, differences for individual queries often help identify where annotations in an index are unhelpful or being ineffectively utilized. This also helps identify bugs, including cases where computed metrics are strong, but \emph{not} because retrieval effectiveness and/or efficiency are strong.\footnote{Based on a true story. Or three.} Fortunately, evaluation frameworks such as PyTerrier\footnote{https://pyterrier.readthedocs.io/en/latest} provide easy access to query-specific differences between models.  












% Tradeoffs
\paragraph{Performance Metric Trade-Offs.}
In addition to considering whether differences in a single metric are consistent, it is important to consider the tradeoffs that occur between effectiveness and efficiency discussed earlier: for example, index sizes and mean retrieval times may increase as more complex information is used for indexing and ranking. There are also well-known trade-offs between effectiveness measures. The classical example is the tradeoff between \emph{recall} and \emph{precision}. The more results that we return, the more likely that recall increases, while the precision of returned results decreases. In theory, we could always return the entire collection for all queries, obtaining a recall of 100\% because all relevant items in the collection are returned for every query. However, for a large collection the average query precision will be very close to 0\%, because few/none of the returned sources are relevant for each query. 

There is a tension amongst other performance measures as well. For example, maximizing mean reciprocal rank (\ie the query-averaged value for one over the rank of the first relevant hit ($\frac{1}{r}$)) or $precision@1$ (\ie the percentage of queries with a relevant source returned at the first position) can lead to reductions in metrics characterizing full ranked results such as mean average precision ($mAP$) or normalized discounted cumulative gain ($nDCG$).



\section{Formula search} 
\label{FormulaSearchEval}


Formula search is one of the common tasks in math information retrieval. A user might search for a formula to see where else it appears in the paper, or a user might want to search over their query logs to find a formula they have previously searched for. The formula search task can be defined as: 

%% TASK TABLES: 
\ourtable
	{!t}
	{
		\scriptsize	
		\begin{tabular}{p{1.15in}   p{0.8in} p{0.8in} p{0.75in} p{0.75in} p{0.75in} }
		
		\toprule
		\textbf{Task \& }		  		&  \textbf{Collection of}	&		&		& \textbf{Effectiveness}\\
		\textbf{Test Collection}	& \textbf{Sources} & \textbf{Queries} & \textbf{Results} & \textbf{Metrics}\\
		\hline
		
		~\\
		\multicolumn{5}{l}{ {\bf Formula Search} }\\
		\midrule

		NTCIR-10 \hfill(2013)	& 	arXiv papers 	 &  Organizers$^w$ & 	F in paper & mAP, P@\{5,10,hit\}\\
		NTCIR-11 \hfill(2014)	& 	Wikipedia		 &  Individual Wiki \linebreak F (known item) 	& F in articles & mRR\\
		NTCIR-12 \hfill(2016)	& 	Wikipedia$'$ & \mbox{Organizers}$^w$ &  F in articles 		& P@\{5,10,15,20\}, Bpref\\

		\hline
		ARQMath-1 \hfill(2020)	& 2018 MSE As & 2019 MSE Qs 	& F in MSE As & nDCG$'$, mAP$'$, P$'$@10 \\%\emph{*Contextualized}\\
		ARQMath-2 \hfill(2021)	&  	& 2020 MSE Qs 	& 	 &  \\%\emph{*Contextualized}\\
		ARQMath-3 \hfill(2022)	& 	 & 2021 MSE Qs 	& 	 &  \\%\emph{*Contextualized}\\
		\hline
		\underline{AccessMath}$^\dagger$ \hfill (2018) & \mbox{Videos +} \LaTeX{}~notes & \mbox{Image~region} \linebreak or~\LaTeX{} & Image regions or \LaTeX{} form. & R@10, mRR@10\\
		%\midrule
		
		~\\
		\multicolumn{5}{l}{ {\bf Math-Aware Search (Ad-Hoc Retrieval)  } }\\
		\midrule
		MREC 	\hfill(2011) 	& arXiv papers 		& $--$ & $--$ & $--$\\
		CUMTC 	\hfill(2015) 	& \mbox{arXiv papers} \linebreak (MREC data) & MathOverflow Qs & Papers & mAP\\
		\hline
		NTCIR-10 \hfill(2013)	& arXiv papers & Organizers$^w$ & Papers & mAP, P@\{5,10,hit\}\\
		NTCIR-11 \hfill(2014)	& \mbox{arXiv frags.} & Organizers$^w$ & Paper frags. & mAP, P@\{5,10,hit\}, Bpref\\
		NTCIR-12 \hfill(2016)	& \mbox{1. arXiv frags.} \linebreak 2. Wikipedia$'$ & \mbox{1. Organizers$^w$} \linebreak \mbox{2. Organizers$^w$} & \mbox{1. Paper frags.} \linebreak \mbox{2. Wiki articles} & P@\{5,10,15,20\}\\
		\hline
		ARQMath-1 \hfill(2020)	& 2018 MSE As & 2019 MSE Qs & F in MSE As &  nDCG$'$, mAP$'$, P$'$@10 \\%\emph{*Contextualized}\\
		ARQMath-2 \hfill(2021)	&  & 2020 MSE Qs & 	 &  \\%\emph{*Contextualized}\\
		ARQMath-3 \hfill(2022)	&  & 2021 MSE Qs &  	&  \\%\emph{*Contextualized}\\
		\underline{Cross-Math}$^\dagger$ \hfill (2024)	&  & \mbox{ARQMath 1-3 Qs} (4 languages) & 	  & P$'$@10, nDCG$'$@10\\
		%\midrule
		
		~\\
		\multicolumn{5}{l}{{\bf Reference Retrieval for Theorem Proving}} \\
		\midrule
		\mbox{NATURALPROOFS} \linebreak (2021) & \mbox{Proof references:} ProofWiki, \linebreak Stacks, Textbks.  & Theorem	& \mbox{Ref set/sequence} in proof & mAP, R@k, edit distance, BLUE\\
		\bottomrule		
		\end{tabular}\\
		\scriptsize
		\textbf{F:} Formula; \textbf{As}: Answers; \textbf{Qs}: Questions; \textbf{MSE:} Math Stack Exchange
		\linebreak
		$^w${\textbf{Wildcard symbols} in at least some query formulas} 
		\linebreak
		 $^\dagger$Cross-modal or cross-language retrieval; \textbf{frags.}: Fragments (roughly paragraphs)
	}
	{Math Search Tasks and Test Collections. Given a query, search systems consult a collection of sources and communicate ranked sources as output.}
	{tab:tasks-sources}


\textit{For the input formula query, find the relevant formulas in the collection of documents.}






While the task is almost defined as the same across different test collection, the relevance definition has evolved. There are two common approaches for defining a relevant formula in this task: 1) formulas that share structural similarity to the query (isolated formula search), and 2) formulas within the same context as the query (contextual formula search). We will next explain the test collections for formula search task and explain how relevance definition has changed:

\textbf{MREC:} The attempts to create a collection for evaluation of formula search models go back to 2011 when Mathematical REtrieval Collection\footnote{\url{https://mir.fi.muni.cz/MREC/index.html}} (MREC) \citep{livska2011web} was introduced. MREC consists of 439,423 scientific documents from arXiv with more than 158 million formulae with parsed MathML. MREC was a collection without any topics for measuring effectiveness. MREC was mostly used to study the efficiency of formula search systems. 

\textbf{CUMTC:} Four years later, the Cambridge University MathIR Test Collection (CUMTC) \citep{stathopoulos2015retrieval} built on MREC, adding 160 test topics derived from 120 MathOverflow discussion threads. This was one of the early works to bring attention to the math community question-answering websites that will benefit from having real-world topics compared to lab-generated ones. CUMTC topics are selected from sub-parts of questions from the 120 threads. These threads have at least one citation to the MREC in their accepted answer.\footnote{Answer accepted by the user who posted the question.} The majority of topics (81\%) have only one relevant document, and 17.5\% have two relevant documents. 
% To evaluate systems, mean average precision (MAP) is used. 

\textbf{NTCIR:} NTCIR-10~\citep{aizawa_ntcir-10_2013} was the first shared task on math-aware search,
 with the formula search task defined as finding similar formulas for a given formula query. In NTCIR-11~\citep{aizawa_ntcir-11_2014}, the formula search task was optional. This task was a known-item retrieval task, where for each query there was one good known result. NTCIR-12~\citep{zanibbi_ntcir-12_2016} introduces the Wikipedia Formula Browsing (WFB) task with a similar definition as NTCIR-10; Given a collection of Wikipedia articles, retrieve relevant mathematical formulae for a given mathematical formula query.

NTCIR-10 was a pilot task and used 100,000 technical papers from arXiv from mathematics, physics, and computer science with 35.5 million formulae. NTCIR-11 brought attention to using English Wikipedia pages with mathematical formulas for the collection as they were simpler. NTCIR-12 uses 319,689 articles from English Wikipedia with over 590,000 formulae in the corpus. All three test collections use lab-generated topics. In NTCIR-10, 21 formula queries were chosen by the organizers for arXiv papers, of which 18 queries included wildcards and 3 were concrete queries. Wildcard queries contain symbols that may be replaced by variables and/or sub-expressions. For example, in the formula query:
$$
\frac{?f(?v+?d)-?f(?v)}{?d}
$$
there are three query variables: ?f, ?v and ?d. The query matches the argument of the limit in the formula
$$
g'(cx)=\lim_{h\to 0}\frac{g(cx+h)-g(cx)}{h}
$$
by replacing g for ?f, cx for ?v, and h for ?d. \emph{Concrete} queries are complete formulas without wildcards. 
NTCIR-11 has a total of 100 queries, with 59 of them including wildcards, and 41 being concrete queries. These queries are formulas randomly selected from Wikipedia pages and were then modified by injecting query variables.
In the NTCIR-12 Wikipedia Formula Browsing (WFB) task, there were 40 queries, divided into 20 concrete queries and 20 wildcard queries. The wildcard queries were created by replacing one or more sub-expressions in each concrete formula query with wildcards. For example, the query $O(mn\log m)$ also appears as $O(${\bf *1*} $\log$ {\bf *2*}$)$, where {\bf *1*} and {\bf *2*} represent two independent sub-expressions. 


For the pooling process, in NTCIR-10, participating teams could submit up to 100 formula instances per formula query. The highest-ranked formula instances were selected from each submitted run, one rank at a time, until the pool to be judged contained at least 100 unique formula instances, each of which had been highly ranked by at least one system. No pooling was used for NTCIR-11 as it was a known-item retrieval task. In the NTCIR-12, participating teams could submit up to 1,000 results per topic. The top-20 formula instances from each submitted run were pooled.  This instance-based definition of uniqueness sometimes resulted in limited diversity in the judgment pools.  As the most extreme example, for the NTCIR-12 WFB query $\beta$ (a short formula consisting of a single symbol), every formula instance in the pool of formulas to be judged was $\beta$.

Both NTCIR-10 and -12 test collections considered three relevance degrees for assessment: Relevant (R), Partially Relevant (P), or Non-relevant (N). For NTCIR-10, the assessors were mathematicians or math students. They viewed each formula instance from the judgment pool in isolation, considering the query-specific scenario and judgment criteria that had been specified when the query was created. For the NTCIR-12 WFB task, there were two groups of assessors; each group independently judged each pooled formula. One group consisted of computer science graduate students, the other consisted of computer science undergraduates. The pooled formula instances were shown to the assessors in context (highlighted in the text where they had appeared in the collection), but assessors were not asked to interpret the pooled formula in that specific context; the assessment was to be done based on the pooled formula itself, with reference to the scenario and relevance criteria that were provided to the assessor with that query. For each topic in NTCIR-11, the single Relevant (R) formula instance was defined as the formula instance that had been used as the formula query.  Note that there may have been other instances of the same or similar formulas in the collection, but like all instances of other formulas, they would be scored as Non-relevant (N).

Per evaluation protocols, NTCIR-10 and -12 combined 3-level judgments from two assessors to form a 5-level ``Aggregate'' relevance judgment for each assessed document. This was done by mapping N to 0, P to 1, and R to 2, and then summing the two scores.  The resulting integer scores ranged from a low of 0 (both assessors judged N) to a high of 4 (both assessors judged R). For computing evaluation measures, these 0 to 4 levels are binarized by treating relevance grades 0, 1, and 2 as non-relevant and treating 3 and 4 as relevant. NTCIR-10 reported P@5, P@10, P@hit (i.e., for all returned results), and MAP. The NTCIR-12 uses P@k for k = \{5, 10, 15, 20\}. Later, researchers used bpref \citep{buckley_retrieval_2004} a preference-based measure designed for incomplete relevance judgments to deal with unevaluated formulas. NTCIR-11 uses mean reciprocal rank (MRR) suitable for known-item retrieval tasks.


\textbf{ARQMath:}  Answer Retrieval for Question on Math (ARQMath) is the most recent attempt to develop a test collection for math information retrieval with a \textit{contextualized} formula search task. ARQMath test collection was developed through three years of CLEF labs, generating test collections referred to by ARQMath-1 (2020), ARQMath-2 (2021), and ARQMath-3 (2022). 

ARQMath collection relies on a math community question-answering website, Math Stack Exchange (MathSE). On this platform, users can post questions and answers. The benefit of using such a collection is having a diverse set of topics in terms of math knowledge, ranging from simple questions from high school to more advanced topics in math. The formula search task in this dataset is defined as: For a given formula inside a math question, find the relevant formulae inside other questions and answers. Table \ref{tab:formulacontext} shows an example query, B.4 in ARQMath-1 (shown in blue), with relevant (shown in green) and non-relevant (shown in red) retrieved formulas. 

In ARQMath, all the questions and answers posted from 2010 to 2018, are provided in collection. Topics were then selected from formulas appearing in questions posted in 2019 (ARQMath-1), 2020 (ARQMath-2), and 2021 (ARQMath-3). To make topics diverse, ARQMath introduced a complexity task for formulas, dividing them into low, medium, and high-complexity topics.  Table \ref{tab:query-complexity} summarizes the number of topics based on complexity in ARQMath test collection, compared to the NTCIR -10 and -12. Note that ARQMath provides additional topics for training.


One of the issues with previous test collections was that, for some queries, there were low numbers of unique assessed formulas. ARQMath pooling is based on visually distinct formulas to have more diverse assessed formulas.
When two formulas have identical symbolic representations, they are defined as \emph{visually identical}, and otherwise as \emph{visually distinct}. Symbolic identity was defined as identical Symbol Layout Trees, as represented by Tangent-S~\citep{davila_layout_2017}, when both were parsable, or identical \LaTeX~strings otherwise. Table \ref{tab:visually-identical} illustrates this distinction by providing examples of visually identical formulas with different \LaTeX~representations. With different pool depths in each ARQMath test collection, the 5 instances contributed to the pools by the largest number of runs were selected for each candidate formula, and ties were broken randomly. 

For assessment, ARQMath organizers hired undergraduate students in mathematics and trained them for assessment. These assessors were trained with a math professor during three training sessions, after each discussing their choice and aiming to minimize assessment errors. Relevance judgment was defined for these assessors as follows:

\textit{For a formula query, if a search engine retrieved one or more instances of this retrieved formula, would that have been expected to be useful for the task that the searcher was attempting to accomplish?}

\ourtable
{!t}
{
% We need to use command Verb, not verb!! (Solved)
\begin{small}
{
\resizebox{\columnwidth}{!}{
\begin{tabular}{c l l }
\toprule
\sc Score~ & \sc Rating & \sc Definition\\
\midrule
3 & High & Just as good as finding an exact match to the formula query would be\\
2 & Medium & Useful but not as good as the original formula would be \\
1 & Low & There is some chance of finding something useful\\
0 & Not Relevant ~~& Not expected to be useful    \\
\bottomrule
\end{tabular}
}
}
\end{small}
}
{Relevance scores, ratings, and definitions for ARQMath formula search task.}
{tab:arqmath-task2-relevance}

Assessors were presented with formula instances, and asked to decide their relevance by considering whether retrieving either that instance or some other instance of that formula would have been useful, assigning each formula instance in the judgment pool one of four scores as defined in Table \ref{tab:arqmath-task2-relevance}. 
For example, if the formula query was ${\sum{\frac{1}{n^{2+\cos{n}}}}}$, and the formula instance to be judged is ${\sum_{n-1}^\infty {1 \over n^2}}$, the assessors would decide whether finding the second formula rather than the first would be expected to yield good results. To do this, they would consider the content of the question post containing the query (and, optionally, the thread containing that question post) to understand the searcher's actual information need. Thus, the question post fills a role akin to Borlund's simulated work task~\citep{pia2003iir}, although in this case the title, body, and tags from the question post are included in the topic and thus can optionally be used by the retrieval system. The MathSE question post was used in place of the scenarios that had been provided with NTCIR-10 and NTCIR-12 queries; no query-specific relevance judgment criteria were provided. The assessor can also consult the post containing a retrieved formula instance (which may be another question post or an answer post), along with the associated thread, to see if in that case the formula instance would indeed have been a useful basis for a search.  Note, however, that the assessment task is not to determine whether the specific post containing the retrieved formula instance is useful, but rather to use that context as a basis for estimating the degree to which useful content would likely be found if this or other instances of the retrieved formula were returned by a search engine.

ARQMath organizer have acknowledged that they did make one potentially noticeable change to the way this relevance definition was interpreted for ARQMath-2 and -3. ARQMath-1 assessors had been instructed during training that if the query and candidate formulas were the same (in appearance), then the candidate was certainly highly relevant. For ARQMath-2 and -3, the interpretation of `exact match' was clarified to take the formula semantics and context directly into account, even in the case of identical formulas (so for example, variables of different types would not be considered the same, even if variable names are identical). This means that an exact match with the formula query may in some cases (depending on context) be considered not relevant. This change may affect the utility of some ARQMath-1 relevance judgments for training systems that will be evaluated using ARQMath-2 or -3 relevance judgments. For example, for the formula query $x^n+y^n+z^n$ (B.289 from ARQMath-2) $x$, $y$, and $z$ could be any real numbers in the original question post in which that formula had originally appeared. The assessors considered all exact matches in the pooled posts in which $x$, $y$, and $z$ referred not to real numbers but specifically to integers as not relevant. On the other hand, formulas that do not share the same appearance or syntax as the query might be considered relevant. This is usually the case where they are both referring to the same concept. For the formula query $\frac{S}{n} \ge \sqrt[n]{P}$ (ARQMath query B.277), formula $\frac{1+2+3+...+n}{n}\geq \sqrt[n]{n!}$ has medium relevance. Both formulas are referring to the AM-GM inequality (of Arithmetic and Geometric Means). 

For each candidate formula, up to five instances of that formula (based on pooling protocols) were then shown to the assessors. Figure \ref{fig:turkle} shows the Turkle\footnote{\url{https://github.com/hltcoe/turkle}} interface used for assessment in ARQMath. As shown in the left panel of the figure, the formula query $\sum_{k=0}^{n} \binom{n}{k} k$ was highlighted in yellow. The assessors could use the question context to understand the user's information need. In the right panel, two instances of one visually-distinct formula, $\sum_{k=0}^{n} \binom{n+k}{k}$, are shown in two different posts. For each instance, the assessor could consider the post in which the instance appeared when deciding the relevance degree. The relevance score for a formula to be the maximum relevance score for any judged instance of that formula.  This relevance definition essentially asks ``if instances of this formula were returned, would we reasonably expect some of those instances to be useful?'' While the official evaluation is done on the visually distinct formulas, ARQMath introduced the concept of ``Bigger Qrel Files'', where more details on assessment is provided. In those file, not only the assessment for each instance of formulas is available, but the assessor IDs are also provided. This can be used to study effectiveness of formula search models, under assessment of different people.  



Finally, evaluation is done after removing duplicate instances and calculating effectiveness measures over visually distinct formulas. This is done by replacing each formula instance with its associated visually distinct formula, and then removing deduplicates from the top of the list downward. ARQMath evaluation measures were different from previous test collections.  One risk when performing a new task for which rich training data is not yet available is that a larger than a typical number of relevant hits may be missed.  Measures that treat unjudged documents as not relevant can be used when directly comparing systems that contributed to the judgment pools, but subsequent use of such a new test collection can be disadvantaged by treating unjudged documents (which, as systems improve, might be relevant) as not relevant. ARQMath, therefore, chose the nDCG$^\prime$ measure (read as ``nDCG-prime'') introduced by Sakai~\citep{sakai_alternatives_2007} as the primary measure. The nDCG measure on which nDCG$^\prime$ is based is widely used when graded relevance judgments are available. ARQMath also uses two other measures: Mean Average Precision (MAP$^\prime$), and Precision at 10 (P$^\prime$@10), after removing the unjudged hits. For MAP$^\prime$ and P$^\prime$@10 High+Medium binarization is used, meaning only the high and medium relevant degrees were considered as relevant.  

%%
%% We need somewhere to point out to the benefit of using primes, for faster evaluation of pilot systems and ideas, where is there is no need to rank the whole collection
%%
Summary of participating teams and runs for NTCIR and ARQMath
As seen in this section, there are different test collection for formula search. Throughout time, the definition of formula search task stayed unique as finding relevant formulas for a given formula query. However, the relevance definitions, evaluation protocols, and collections have changed. One other factor that can contribute to diversity of assessed instances in these test collections, in the number of participating teams in the shared tasks. Table \ref{tab:formula-search-teams} summarizes the number of runs that were pooled in each of the formula retrieval test collections. 






\section{Math-aware search}%: Tasks and Evaluation}


A math-aware search engine refers to a search engine that supports retrieval using both formulas and keywords. Unlike regular web searches, it goes beyond just text and understands the meaning encoded within mathematical symbols and formulas. We can formalize the math-aware search task as follows:

\textit{Given a query combining text and a formula, find relevant documents.}

This task distinguishes itself from isolated and contextualized formula search tasks by the nature of the information need. In the latter tasks, the information need solely revolves around the formula itself, and the retrieved items are also formulas. In contrast, the math-aware search task leverages both text and formula to express a mathematical information need, ultimately aiming to find relevant documents. This ranges from simple ad-hoc query ``$a^2+b^2=c^2$ proof'' to full math question. Similar to formula search, the main standard test collections for this task are the NTCIR and ARQMath shared tasks for math-aware search, which we will discuss next.




\textbf{NTCIR:} NTCIR-10, -11, and -12 used similar collections as formula search task, consisting of arXiv and Wikipedia. The retrieval unit in NTCIR-10 is the full document, which can make assessment challenging. Therefore, in NTCIR-11, the retrieval unit is reduced paragraphs, resulting in 8,301,578 search unit. NTCIR-12 relies on existing NTCIR-11 arXiv collection, and for Wikipedia pages, the retrieval unit is the full page.

NTCIR test collections contain different number of topics, growing in each lab. In NTCIR-10, there are 15 assessed formula+text topics. NTCIR-11 contains 50 topics, where each has at least one keyword and one formula. In NTCIR-12, topics were developed for search on two different collections: arXiv and Wikipedia. 29 arXiv and 30 Wikipedia topics were assessed. All the topics contained at least one formula, but 5 in the arXiv and 3 in the Wikipedia set had no keywords. All the NTCIR topics are lab-generated and only the query is provided with no additional description of information needs and search scenario.

For pooling, NTCIR-10 follows its formula search task approach, with each team submitting up to 100 documents per topic, and picking top-ranked documents until 100 documents are gathered for each topic. Each team in NTCIR-11 formula+text search task was allowed to submit up to 4 runs, returning the top-1000 results per query. For each topic, 50 retrieval units were chosen from the union of the retrieval results. In NTCIR-12, the top-20 ranked results per run were included in the pool for assessment.

The assessment process in NTCIR-10 for text+formula searches was similar to the formula search task, with the same assessors. The relevance was decided based on the retrieved formula, not the document due to high number of formulas in documents, and having whole document as the retrieval unit. For each formula, the assessors were asked to select either relevant (R), partially-relevant (PR), or not relevant (N). Each formula was assessed by one or two assessors. In NTCIR-11, the assessors were shown the title of the topic, the relevance description, and an example hit (if any) as supplementary information. In this collection, in contrast to NTCIR-10, the relevance was assessed not on a formula basis, but a retrieval unit basis. That is to say, the assessors judged the relevance of each retrieval unit to the query based on the keywords, as well as the formulas included in the submission files. To make sure that assessors are familiar enough with math, they were chosen from third-year undergraduate and from graduate students in mathematics. The relevance levels were similarly defined in NTCIR-12, however, the assessors for Wikipedia topics were computer science students. Each hit was evaluated by one undergraduate and one graduate student. The overall judgement in all NTCIR test collections was decided as R/R and R/PR as relevant, PR/PR, R/N, PR/N as partially-relevant, and N/N as not relevant. 

As for the evaluation measures, NTCIR-10 has MAP, P@\{5,10, hit\} as four basic measures. In NTCIR-11, in addition to MAP and P@\{5, 10\}, bpref was also included to handle unjudged instances. NTCIR-12 tasks reported P@\{5, 10, 15, 20\}. In all cases, relevance judgments for formula instances that were missing from the pools (as can happen for P@hit and MAP) were treated as not relevant.

\textbf{ARQMath:} ARQMath main task is answer retrieval for math questions. This is motivated by the query log analysis on math searched \citep{mansouri_characterizing_2019}, where it was shown that the number of question queries are almost 10\% higher in math compared to general searches.  The task is defined as:

\textit{Given a new mathematical question (not seen in training) find the relevant answers to it.}

ARMath was built on Math Stack Exchange, as shown in Figure \ref{fig:ARQMath}. All the questions and their related answers posted from 2010 to 2018 are provided for training. The ARQMath collection contains roughly 1 million questions and 28 million formulas. ARQMath topics are selected from the new questions posted in 2019, 2020, and 2021. The main constraint for selecting topics was that the question post should contain at least one formula.

\ourfigscaled
	{!t}
	{0.7}
	{figures/Evaluation/ARQMathMathSE}
	{ARQMath Answer Retrieval task built on Math Stack Exchange. Questions and their answers posted from 2010 to 2018 are available for training purposes. Topics are selected from the new questions and answers should be retrieved from the answers given to old questions.}
	{fig:ARQMath}

Overall, 226 assessed topics are produced for testing in ARQMath with 77 in ARQMath-1, 71 in ARQMath-2, and 78 in ARQMath-3. When choosing topics, 3 kinds of categories were considered. The first category was based on their type (topic). The organizers labeled each question with one of three broad categories, \textit{computation}, \textit{concept} or \textit{proof}. Topics were also categorized based on their perceived difficulty level into three categories of low, medium, and high. The last categorization was based on whether a topic is dependent on text, formulas, or both. Figure \ref{fig:ARQMathTopics} shows counts of topics per category in ARQMath-1, -2 and -3.

The pooling process in ARQMath test collections are based on different cuts of participating teams. Each team was allowed to submit up to 5 runs, selecting one run as primary and the others as alternative. Deeper cuts were considered for primary runs. 

ARQMath assessor for answer retrieval task were also selected from students in mathematics, similar to the formula search task. There were 2-3 training sessions with a math professor to introduce the task and train the assessors in each test collection. Some questions might offer clues as to the level of mathematical knowledge on the part of the person posing the question; others might not. To avoid the need for the assessor to guess about the level of mathematical knowledge available to the person interpreting the answer, we asked assessors to base their judgments on the degree of usefulness for an expert (modeled in this case as a math professor) who might then try to use that answer to help the person who had asked the original question. Four relevance degrees are considered for this task, defined in Table \ref{tab:ARQMathTask1Relevance}. Finally, for evaluation, the same evaluation measures as the formula search task were used: nDCG$^\prime$, MAP$^\prime$ and P$^\prime$@10.

\ourtable
{!t}
{
% We need to use command Verb, not verb!! (Solved)
\begin{small}
{
\resizebox{\columnwidth}{!}{
\begin{tabular}{c l p{3.6in} }
\toprule
\sc Score~ & \sc Rating & \sc Definition\\
\midrule
3 & High & Sufficient to answer the complete question on its own \\

2 & Medium & Provides some path towards the solution. This path might come from clarifying the question, or identifying steps towards a solution \\

1 & Low & Provides information that could be useful for finding or interpreting an answer, or interpreting the question  \\

0 & Not Relevant & Provides no information pertinent to the question or its answers. A post that restates the question without providing any new information is considered non-relevant \\
\bottomrule
\end{tabular}
}
}
\end{small}
}
{Relevance assessment criteria for the ARQMath Answer Retrieval task.}
{tab:ARQMathTask1Relevance}

To summarize, NTCIR and ARQMath test collections are commonly used for evaluating math-aware search systems. With the pilot task started at NTCIR-10, more and more was learned about developing math-aware test collections. For instance, starting in NTCIR-10, the retrieval units were the whole document, which made assessment hard, and that was reduced to paragraphs in NTCIR-11. With observation in NTCIR-11 and using Wikipedia as a simpler collection, NTCIR-12 used both arXiv and Wikipedia as the collection.

NTCIR topics were all lab-generated. ARQMath, however, considered math questions posted by real-world users on Math Stack Exchange as topics. Topics were selected based on different categorizations to ensure diversity. ARQMath brought attention to prime effectiveness measure to handle unjudged answers which makes comparison fair for the future systems that did not participate in the pooling process. This approach can also be useful for pilot study of less efficient systems, and ranking the whole collection can be time-consuming. These systems can only re-ranked the assessed answers. ARQMath provides all the runs that participated in the pooling process, which can provide a means of studying the effectiveness of different approaches and understanding their strengths and weaknesses. Table \ref{tab:mathaware-search-teams} summarizes the math-aware test collections, their collections, and the number of teams and runs participating in building them.



\textbf{Math Conversational Search:} With advances in conversational search, these models are explored for math as well. MathBot~\citep{grossman2019mathbot} is a text-based tutor capable of explaining math concepts providing practice questions and offering feedback to the students. Compared to other domains, there are no standard benchmarks developed for evaluating math conversational search systems. The use of clarifying questions for math has been studied on Math Stack Exchange by extracting comments on math questions~\citep{10.1145/3578337.3605123}. Tasks such as generating clarifying questions, and detecting ambiguous math queries can be studied on this dataset.   

\textbf{Cross-Lingual Math Information Retrieval:} Current math search engines and test collections are primarily developed for the English language, limiting their accessibility and inclusivity. Cross-lingual math information retrieval (CLMIR) is a new task, focusing on retrieving mathematical information across languages. CLMIR has been explored for math-word problems \citep{tan-etal-2022-investigating}, where existing datasets were translated into Chinese using online machine translators, and manually refined the translations. CrossMath~\citep{gore2024crossmath} is a novel CLMIR test collection comprising manually translated topics in four languages (Croatian, Czech, Persian, and Spanish). These are the same topics used in the ARQMath Answer Retrieval task. This domain is fairly new and a research gap to be filled. There are approaches proposed for machine translation of mathematical text~\citep{9369381, petersen-etal-2023-neural} and more to come in the future.





%: MATH QUESTION ANSWERING
\section{Math question answering}

% Myriad items here (see table and text)
% + Evaluation

\paragraph{Evaluating Answers.}


\textbf{Math Question-Answering:} This problem is defined as generating or extracting answers to math questions. This is different from ARQMath's answer retrieval task, where the answers are retrieved from human-written content, with no further changes. The SemEval 2019, Task 10 \citep{hopkins-etal-2019-semeval} provides question sets from MathSAT (Scholastic Achievement Test) practice exams in three categories: Closed Algebra, Open Algebra, and Geometry. The majority of the questions were multiple choice, with some having numeric answers. This test collection contains 3860 questions, of which 1092 are used as the test set. The accuracy measure is used as an evaluation metric for this task, as the systems choose the answer from a set of choices.

%:%%%%%% QA no sources
\ourtable
	{!t}
	{ 		
		\scriptsize	
		\begin{tabular}{l  p{1.25in} p{1in} p{0.75in} }

		\toprule
		\textbf{Task \& }	&	   		&		&		 \textbf{Effectiveness}\\
		\textbf{Test Collection} & \textbf{Queries} & \textbf{Results} & \textbf{Metrics}\\
		\hline

		~\\
		\multicolumn{4}{l}{ {\bf Math Problems} }\\
		\midrule
		Dolphin18k \hfill(2016) 	  & Arithm./algebra WP$^\dagger$ & Number set & Accuracy$^\circ$\\ 
		AQuA-RAT \hfill(2017) & MC$^\triangle$ WP& \mbox{Rationale} \linebreak \mbox{+ chosen answer} &	Accuracy, \linebreak Perplexity, \linebreak \mbox{Expert ration.} \linebreak{\mbox{+ BLEU}}\\

		SemEval \hfill (2019)	 	&  \mbox{WP} (SAT questions) 	& \mbox{Numeric or} \linebreak chosen answer	& Accuracy\\
		MathQA \hfill (2019)		  & MC WP	      &  \mbox{Rationale} \linebreak \mbox{+ chosen answer} & Accuracy\\
		ASDiv \hfill (2020)		  & WP		& Equation and value & Accuracy\\
		MATH \hfill(2021) 	 & WP 	& \mbox{Step-by-step soln}  \linebreak \mbox{+ final answer} 	&  Accuracy \\
		GSM8k \hfill (2021)		  & WP & \mbox{Step-by-step soln} \linebreak \mbox{+ final answer} & Accuracy\\ %test@1\\
		\hline
		DROP \hfill(2019) 		 & Paragraph questions & \mbox{Number, entity, etc.} & Accuracy, F1,EM\\%EM$^\ddagger$, F1\\
		% LILA \hfill(2022) 	 	& ???			& Python program with answer value & Annotated solution program, target value; F1 score measured how??\\

		
		


		~\\
		\multicolumn{4}{l}{{\bf Math Problems with Graphical/Visual Content }} \\
		\midrule

		GeoQA \hfill (2021)  & \mbox{MC geometry problems} \linebreak w. diagram & Chosen answer & Accuracy \\
		UniGeo \hfill (2022)  & \mbox{MC w. diagram} \linebreak \mbox{~~}(GeoQA extension) & Chosen answer & Accuracy\\

		\hline
		MathVista \hfill (2023)  & Figure QA, WP, geometry problems, textbook questions, VQA & \mbox{Chosen answer or} numeric  & Accuracy\\
		Math-Vision \hfill (2024)  & Math reasoning with visual elements & \mbox{Step-by-step soln} \linebreak \mbox{+ final answer} & Accuracy\\ 
		\hline
		TabMWP \hfill (2023)	 & MC w. tabular data  & Number or  text &  Accuracy\\
		
		~\\
		\multicolumn{4}{l}{\bf Open Response}\\%: QA \& Turn-Based Conversational Problem Solving}}\\
		\midrule
		ARQMath-3 \hfill (2022) & ARQMath-3 MSE Qs 	& \mbox{Written response} \linebreak \mbox{(formulas + text)} & \mbox{Relevant MSE} \mbox{~~}answers, \linebreak \mbox{+ token F1,} \linebreak+ BERTScore\\
		\hline
		MathDial \hfill (2023)  & \mbox{LLM-simulated student} \linebreak \mbox{Q. or comment} \linebreak  \mbox{~~}(GSM8k questions) & \mbox{Responses to Q.} \linebreak and comments & \mbox{Expert resp.} \linebreak \mbox{+ sBLEU,} \linebreak \mbox{+ BERTScore}\\
		\bottomrule
		
		\end{tabular}\\
		\scriptsize
		
		 $\dagger$\textbf{Word Problems}; $^\circ$\textbf{Accuracy} = test@1 = \% correct $\approx$ Exact Match (EM)  
		 \linebreak $^\triangle$\textbf{Multiple Choice}%; $\ddagger$Exact Match
	}
	{Math Question Answering (QA) Tasks and Test Collections. Given a query, QA systems communicate one answer. Answer formats include written responses, computer programs, values (\eg numbers, lists), and multiple choice alternatives (\ie classification). Many queries come from standardized math aptitude tests, such as the SAT.}% (EM: Percent of Exact match different accuracy, the number of correctly answered questions.)}
	{tab:collections}


More diverse datasets have been introduced since SemEval task, focusing on mathematical reasoning. DROP (Discrete Reasoning Over the content of Paragraphs) dataset \citep{dua2019dropreadingcomprehensionbenchmark} is known as a reading comprehension task where a for given paragraph and questions, the system should obtain the correct solution by reasoning. This dataset has been commonly used for evaluating reasoning capabilities of large language models such as Gemini and PaLM. The MATH dataset~\citep{hendrycks2021measuringmathematicalproblemsolving} is another math question-answering dataset, developed on mathematics competitions such as
AMC 10, AMC 12, and AIME. This dataset provides more advanced questions in math with 12,500 problems (7,500 training and 5,000 test). The problems in datasets are labeled with difficulty levels from 1 to 5 and are categorized into seven groups: Prealgebra, Algebra, Number Theory, Counting and Probability, Geometry, Intermediate Algebra,
and Precalculus. Answers in this dataset, include step-by-step solution, making it suitable for training models to provide explanations for their answers. Datasets such LILA \citep{mishra-etal-2022-lila} are developed to unify mathematical reasoning benchmark. LILA extends 20 existing datasets  to include a solution program (not only the answer), and instruction annotations to enable instruction-based learning. Answers are represented as Python strings that prints a number, expression, list, or other data format. For each task in this collective dataset, instruction annotations are provided with a clear definition of the task, a prompt providing a short instruction and examples to help learning by demonstration. The systems' effectiveness is usually measured through F1-Score comparing the models' output against gold answer.



ARQMath-3 \citep{10.1007/978-3-031-13643-6_20} introduced a pilot domain question-answering task using the same topics as the math-aware search task. Evaluation measures for this task used lexical overlap of tokens (viewing answers as a bag of tokens), using $F_1$ score between the system's answer and relevant answers from the answer retrieval task. The maximum $F_1$ score across all the relevant answers is considered the final score. With a similar approach, BERTScore~\citep{zhang2020bertscoreevaluatingtextgeneration} is also used to measure this overlap.


\textbf{Math-word Problem (MWP):} Automatically solving math word problems has been an area of interest for artificial intelligence scientists for a long time~\citep{feldman1995gw}. This is basically a math question written in words instead of numbers and equations. Table \ref{tab:mathwordproblem} shows simple examples of the math word problem. 
There are a diverse number of datasets for this task. Earlier datasets such as Dolphin18K \citep{huang-etal-2016-well} have focused on arithmetic and algebraic problems, with solutions provided only in the form of equations or final answers. MathQA \citep{amini-etal-2019-mathqa} contains 37k English multiple-choice math word problems built on AQuA-RAT \citep{ling-etal-2017-program}, which was reportedly suffering from poor annotation, including wrong solutions and problems that could not be solved without brute-force enumeration of solutions. 

Despite the correction to the AQuA-RAT dataset, around 30\% of MathQA solutions had inconsistencies. Moreover, the diversity of questions is a big issue that can affect how correctly systems are evaluated. ASDiv (Academia Sinica Diverse MWP Dataset) \citep{miao-etal-2020-diverse} contains 2.3K math word problems; however, each question is labeled with a problem type (e.g., Basic arithmetic operations, Aggregative operations) and grade level to show the difficulty level of the problems. This dataset provided different diversity metrics which helped the development of future datasets. For example, GSM8K \citep{cobbe2021trainingverifierssolvemath} consists of 8.5K school math problems created by human problem writers, with 1K problems as the test set. These problems need 2 to 8 steps to get to the solution, using primary calculations with basic math operations to find the answer. This dataset contains questions that need basic knowledge, such as the number of days in a week. 

While there are many math-word problem with textual data, in recent years there have been attempts to study this area with multimodal data. For example, TabMWP \citep{lu2023dynamicpromptlearningpolicy}, contains 38K open-domain grade-level problems that require mathematical reasoning on both textual and tabular data. To solve these problems, systems need to look into the textual data and look up into the given table cells. Visual math question-answering discussed later in this section is also another multimodal math question-answering problem. 

Math word problem, is the most basic category of more broad domain of study, \textit{mathematical reasoning}. We have visited math question answering and math-word problem as two sub-categories of this broader problem. Another interesting problem is theorem proving. NATURALPROOFS~\citep{welleck2021naturalproofs} for example, is a multi-domain corpus of mathematical statements and their proofs, written in natural mathematical language. The main tasks in this dataset are: 1) \textit{mathematical reference retrieval}: given a theorem, retrieve a set of references that occur in the theorem proof, and 2) \textit{mathematical theorem generation}: generate the sequence of references that occur in a given theorem's proof.

As AI techniques develop fast, more and more challenging tasks and datasets are being introduced. For example, the MathDial \citep{macina-etal-2023-mathdial} dataset brings attention to math tutoring dialogues by connecting an expert annotator, who role-plays a teacher, with an LLM that simulates the student for reasoning problems. This dataset has 3k tutoring conversations grounded in math word problems from GSM8k.  It consists of one-to-one interactions between human teachers and a Large Language Model (LLM) that simulates student errors. The dataset is designed to capture the nuances of student-teacher interactions in a tutoring setting, focusing on multistep math problem-solving scenarios. The main task in MathDial is \textit{Tutor Response Generation}, aiming at modeling the teacher in a dialogue by generating follow-up turns to guide the student to solve problems. 

The most recent, and ongoing challenge as the time of writing this book is AI Mathematical Olympiad (AIMO).\footnote{\url{https://aimoprize.com/}} The fund aims to promote the open development of AI models that can perform mathematical reasoning, ultimately resulting in a publicly available AI model capable of winning a gold medal at the International Mathematical Olympiad (IMO).

\textbf{Visual Math Question-Answering:} Visual aids such as plots, diagrams, and geometric concepts are commonly used in math. While text-based problems are investigated more extensively, visual math question-answering is still unexplored for the most part. GeoQA \citep{chen-etal-2021-geoqa} is a geometric question-answering dataset, where for a textual description of the problem and its related diagram, systems should choose the correct answer from multiple choices. UniGeo \citep{chen-etal-2022-unigeo}, expanded this dataset, by including the 4,998 calculation problems (from GeoQA) and adding 9,543 proving problems. 

While this was an early attempt at this problem, MathVista \citep{lu2024mathvistaevaluatingmathematicalreasoning} provides 6,141 examples of mathematical and visual tasks and studies several large language models, and large multimodal models.\footnote{https://mathvista.github.io/} These examples focus on five primary tasks including, figure question answering, geometry problem solving, math word problem, textbook question answering, and visual question answering with two categories of multiple-choice and free-form questions. 
Math-Vision \citep{wang2024measuringmultimodalmathematicalreasoning} is another recent attempt at studying large multimodal models for mathematical problems with visual contexts, providing 3,040 diverse problems.



\section{Summary}

While we discussed tasks around search systems in math, it is noteworthy to mention that tasks such as math entity linking \citep{kristianto2016entity} (as discussed in the previous chapter), natural language premise selection (retrieving the premises useful for proving a mathematical statement) \citep{ferreira2020naturallanguagepremiseselection} are other related tasks to explore. Another set of tasks closely related to math information retrieval is the extraction of mathematical formulas from documents. One can view this as a step before indexing, but the outcome of this step can greatly impact the quality of retrieval systems. ICDAR Competition on Recognition of On-line Handwritten Mathematical Expressions (CROHME) considers different tasks such as recognizing formulas from online stroke data and image generated from handwritten strokes \citep{8978036, 10.1007/978-3-031-41679-8_33}. While beyond the scope of this book, these tasks play a crucial role in correctly identifying formulas and passing them to the math retrieval models. 

 

% , reasoning for solving math problems \citep{lewkowycz2022solving} a





==> main-nowbook.tex <==
\PassOptionsToClass {book,biber}{nowfnt}
\input {main}


==> main-nowchapter.tex <==
\PassOptionsToClass {chapter,biber}{nowfnt}
\input {main}


==> main-nowebook.tex <==
\PassOptionsToClass {ebook,biber}{nowfnt}
\input {main}


==> main-nowechapter.tex <==
\PassOptionsToClass {echapter,biber}{nowfnt}
\input {main}


==> main-nowplain.tex <==
\PassOptionsToClass {plain,biber}{nowfnt}
\input {main}


==> main-nowsample.tex <==
\PassOptionsToClass {sample,biber}{nowfnt}
\input {main}

